Fast & Efficient Normalizing Flows and Applications of Image Generative Models

This thesis presents novel contributions in two primary areas: advancing the efficiency of generative models, particularly normalizing flows, and applying generative models to solve real-world computer vision challenges. The first part introduce significant improvements to normalizing flow architectures through six key innovations: 1) Development of invertible 3x3 Convolution layers with mathematically proven necessary and sufficient conditions for invertibility, (2) introduction of a more efficient Quad-coupling layer, 3) Design of a fast and efficient parallel inversion algorithm for kxk convolutional layers, 4) Fast & efficient backpropagation algorithm for inverse of convolution, 5) Using inverse of convolution, in Inverse-Flow, for the forward pass and training it using proposed backpropagation algorithm, and 6) Affine-StableSR, a compact and efficient super-resolution model that leverages pre-trained weights and Normalizing Flow layers to reduce parameter count while maintaining performance. The second part: 1) An automated quality assessment system for agricultural produce using Conditional GANs to address class imbalance, data scarcity and annotation challenges, achieving good accuracy in seed purity testing; 2) An unsupervised geological mapping framework utilizing stacked autoencoders for dimensionality reduction, showing improved feature extraction compared to conventional methods; 3) We proposed a privacy preserving method for autonomous driving datasets using on face detection and image inpainting; 4) Utilizing Stable Diffusion based image inpainting for replacing the detected face and license plate to advancing privacy-preserving techniques and ethical considerations in the field.; and 5) An adapted diffusion model for art restoration that effectively handles multiple types of degradation through unified fine-tuning.

==> Chapters/chapter11.tex <==
\chapter{Determining spin state gap energetics in 3d transition metal complexes using Machine Learning }\label{chap:spin_ml}
\section{Introduction}

Determining accurate spin state gap energies (SSE) in 3d transition metal complexes (TMC) is a longstanding challenge in theoretical chemistry \cite{daku2012,2,3,4,5,6}. Typically, metal complexes involving $d^{4}-d^{7}$ electronic configurations may exhibit different energetically close-lying spin states (high spin, intermediate spin, low spin) depending upon factors like ligand field environment, electron configuration, solvent environment, etc. Although a quantum mechanical phenomenon, spin states can significantly affect large-scale problems like predicting catalytic pathways for homogenous and heterogeneous systems, metalloenzymes, and biomimetic complexes. Additionally, spin state energetics is crucial for designing spin-crossover complexes and other magnetic materials \cite{7,8,9,10,11,12}. There are two ways to obtain experimental SSE \cite{13}, namely, (1) Enthalpy measurements on spin crossover complexes and (2) Spin-forbidden d-d transitions. Unfortunately, experimental data in this domain is scarce. Most relevant intermediates in reaction mechanisms are short-lived, making SSE determination unachievable for such cases. Hence, the determination of SSE through theoretical/computational techniques holds central importance. Recently, Radon and co-workers have developed methods to eliminate the vibrational and environmental effects from experimental gaps to obtain purely electronic SSE, which can serve as a benchmark for theory \cite{13,14,15}.
\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{Images/Fig-Chap9C/figures/Figure1.pdf}
    \caption{Schematic representation of workflow used in this work.}
    \label{fig:overview}
\end{figure}

A wealth of studies have focused on calculating accurate SSE for various complexes. Unfortunately, no single computationally inexpensive theoretical technique is known to produce reliable spin state gaps for systems involving different kinds of metal centers and ligand environments \cite{16,17,18,19,20}. Discrepancies in computed SSEs from different levels of theories arise from the disparate treatment of high spin (HS) and low spin (LS) structures by electronic structure methods, owing to their varying electron correlation. DFT-based methods suffer from the amount of HF exchange present in the exchange-correlation functional \cite{21}, while CASPT2 tends to overestimate HS state stability \cite{5}. Expensive methods like DLPNO-CCSD(T) and CASPT2/CC are promising to improve SSE quality systematically, but such studies are limited to a few Fe SCO complexes \cite{3,22}. It is worth exploring the potential of machine learning (ML) algorithms in addressing this challenge and assessing whether they can offer a cost-effective approach to SSE prediction. However, given the need for adequate datasets, DFT remains the most practical choice for generating the training data.

Earlier studies have successfully devised ML models to predict the ground-state spin of transition metal complexes. Kulik and co-workers \cite{23} devised artificial neural network (ANN) models to predict experimental ground state spins of 2000 unique Fe(II)/Fe(III) complexes based on bond length heuristics of the central metal atom. Corminboeuf’s group \cite{24} has recently applied a modified relative metal radius parameter that can successfully predict ground state spins of 2063 diverse complexes from the Cambridge Structural Database (CSD) \cite{25,26}, irrespective of metal identity (Cr-Ni), coordination geometry, and ligand types. The underlying principle is that high-spin complexes will have a larger metal-ligand bond length (due to the occupation of anti-bonding orbitals) than low-spin structures. However, the prediction of SSE depends upon diverse electronic factors.

Kulik and co-workers \cite{27,28,29,30,31} have developed ML models for SSE prediction based on features like Pauling electronegativity, covalent radii, bond order, ligating atoms and their immediate neighboring atoms, connectivity, and mainly on ligand-specific descriptors along with metal-based descriptors. However, there can be cases where the coordinating environment may be atypical, and ligand-specific descriptors may be incapable of describing the electronic structure properly to yield reasonable SSEs. There is a need to test descriptors independent of name identifiers and beyond heuristic atomic properties. Alternatively, in predicting energetics, ML has been leveraged to use features from cheap quantum mechanical techniques to predict molecule-specific quantities, which can only be obtained through higher-level and expensive \textit{ab initio} computations. Recently, Miller and co-workers \cite{32} tried to adapt feature vectors beyond usual atomic/geometric specifications to predict small organic molecules' MP2 and CCSD correlation energies. They utilized feature vectors involving elements from Fock, Coulomb, and exchange matrices obtained after Hartree-Fock calculations. When trained solely upon H$_2$O, these features could predict CCSD correlation energies for NH$_3$, CH$_4$, and HF with mean errors of 0.5 mH. Poloni’s group \cite{33} recently trained an ANN-based exchange-correlation functional upon calculating electron densities over small molecular fragments like Fe-O, CuF, and Cr-H and predicted spin-state energetics of actual complexes as difficult as Fe(NCH)$_6^{2+}$ and Co(NCH)$_6^{2+}$ \cite{daku2012}.

Our study aims to find ML descriptors to predict SSE and address the aforementioned disparate treatment of HS and LS structures among theoretical methods. It is well known that typically obtaining optimized structures for transition metal complexes for their respective high spin (HS) states using DFT methods tends to be uncomplicated as they are single references in nature \cite{34}. Conducting similar DFT optimizations for the corresponding low spin (LS) states of such molecules can be fraught with convergence issues due to the relatively higher multi-reference nature of such spin states \cite{35}. Our study is essentially a test bed to see if orbital-based non-geometric features yielded by an HS spin state optimization can be leveraged to predict SSEs at the DFT level of theory. Figure~\ref{fig:overview} illustrates the workflow used in this work. Our feature vectors encompass straightforward properties derived from single-point HS DFT calculations, including MO eigenvalues of d-orbitals, natural charges, atomic spectra of bare metal ions (taken from the NIST database \cite{NIST}), and simple identity information of the complexes. The inclusion of zero-field atomic-level splitting as a feature in our descriptor set was inspired by drawing parallels to crystal field theory, where the TM metal complex spin state energetic separation is understood through the prism of how the metal atomic levels split when ligands are brought in the vicinity of it. In this study, we have trained multiple ML models to predict 1434 SSE values for 934 transition metal complexes. Despite training with simple mono-dentate Werner-type complexes, our model exhibits transferability to more complex bi-dentate $\pi$ binding ligands. Moreover, our approach enables rapid SSE determination in a single-step HS calculation, obviating the need for computationally challenging LS optimizations even at the DFT level of theory.


\section{Machine Learning Framework}

In this study, we explored the application of machine learning (ML) algorithms to predict spin state energetics (SSE) using non-geometric, orbital-based features derived from high-spin (HS) single-point DFT calculations. We aimed to circumvent the computational challenges of low-spin (LS) geometry optimizations by leveraging features obtainable solely from HS configurations. To this end, we utilized a diverse set of descriptors encompassing d-orbital eigenvalues, natural population analysis (NPA) charges on the metal and ligand-coordinating atoms, HOMO-LUMO gaps of ligands, and gas-phase atomic-level splittings of the bare metal ions extracted from the NIST database~\cite{NIST}. This novel inclusion of atomic spectroscopy-derived descriptors was motivated by crystal field theory and has not been explored in earlier SSE-focused ML works~\cite{27,28,29,30,31}. Categorical information, such as metal identity, oxidation state, spin multiplicity, and ligand names, was encoded using multiple schemes to enrich the feature space further.

\begin{figure}
    \centering
     \includegraphics[width=1.0\linewidth]{Images/Fig-Chap9C/figures/Figure3.pdf}
    \caption{Description of feature vectors used for training the dataset.}
     \label{fig:fig_3}
 \end{figure}

Three supervised ML models—Polynomial LASSO regression~\cite{LASSO}, Multilayer Perceptron (MLP)~\cite{MLP}, and XGBoost regressor~\cite{XGB}—were trained and evaluated to identify the most effective approach for SSE prediction. Model implementation and training were implemented using the \texttt{scikit-learn} library~\cite{scikit-learn}. The dataset was split into $80\%$  training and $20\% $ testing subsets, with 5-fold cross-validation to ensure robustness. The models were trained using Mean Squared Error (MSE) loss, with hyperparameters such as regularization strength and neural network architecture optimized through grid search. Among the models, the Polynomial LASSO (degree = 2) was particularly effective in capturing nonlinear dependencies while maintaining feature sparsity. Model performance was assessed using standard regression metrics: mean absolute error (MAE), root mean square error (RMSE), and R$^2$ score. To interpret model predictions and identify key contributing features, SHAP (SHapley Additive exPlanations) values~\cite{SHAP} were computed, providing insights into the predictive power of different feature categories.

\section{Results and Discussion}

% \section{RESULTS AND DISCUSSION}

To evaluate the predictive performance of our models, we trained on a dataset comprising 1147 transition metal complexes with spin state energies (SSEs), using a descriptor set (DC-Ref) that integrates electronic structure-based and identity-based features. Among the three models tested, the MLP outperformed LASSO and XGB with the lowest test MAE of 4.0 kcal/mol and an R$^2$ of 0.93, as shown in Table~\ref{tbl:scores}. Although the MLP model does not surpass prior ML benchmarks regarding lowest MAE~\cite{27,30}, it demonstrates the effectiveness of incorporating electronic structure-based descriptors for capturing the underlying physics of spin state energetics. Figure~\ref{fig:fig_4} shows the ligand-wise performance breakdown, revealing that carbonyl complexes have the widest prediction error range, while ligands such as cyanide and acetonitrile yield significantly lower errors. Interestingly, simple ligands like water and ammonia also contribute to larger prediction spans, underscoring the complexity of SSE prediction in systems with diverse ligand field strengths.

\begin{table}[!ht]
\small
  \caption{Training and test MAE, RMSE, R$^2$ scores for different models.}
  \label{tbl:scores}
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{lcccccc}
    \hline
    Model & Train RMSE & Train MAE & Train R$^2$ & Test RMSE & Test MAE & Test R$^2$ \\
    \hline
    LASSO & 3.7	& 2.8 & 0.97 & 6.5 & 4.8 & 0.90 \\
    XGB   & 2.1 & 1.6 & 0.99 & 6.3 & 4.8 & 0.90  \\
    MLP   & 3.0 & 2.3 & 0.98 & 5.2 & 4.0 & 0.93  \\
    \hline
  \end{tabular}
  }
\end{table}

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.90\linewidth]{Images/Fig-Chap9C/figures/Figure4.pdf}
    \caption{Boxplots of the test set MLP SSE prediction error for complexes belonging to specific ligands in the dataset. The $n$ value above the boxplot is the number of complexes belonging to each category.}
    \label{fig:fig_4}
\end{figure*}

To further understand the predictive behavior of the MLP model, we conducted a SHAP-based feature attribution analysis (Figure~\ref{fig:fig_5}), which highlighted the dominance of electronic property features, particularly natural charges and d-orbital energies, over simple identity-based encodings. Notably, the natural charge on the metal center emerged as the most impactful single feature, reinforcing the physical relevance of these descriptors. An error analysis of poorly predicted cases (Figure~\ref{fig:fig_6}) reveals that Fe-based complexes and those with lower spin multiplicities are more prone to higher prediction errors, partly due to their smaller SSE values and higher sensitivity to spin-state energetics. These observations indicate that while our model generalizes well across most of the chemical space, specific subsets, like Fe SCO complexes, present intrinsic challenges due to narrow SSE distributions and low data representation.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.99\linewidth]{Images/Fig-Chap9C/figures/Figure5.pdf}
    \caption{SHAP (SHapley Additive exPlanations) analysis of MLP predictions. The X-axis shows the contribution of each feature in the predictive model. The blue/pink color indicates a feature that pushes the prediction toward a negative/positive direction from the average prediction of $-3.916$. The feature numbers correspond to the following classes: 0–5 (Atomic spectra (DFT)), 6–12 (Natural charges), 13–22 (d-eigenvalues), 23–28 (HOMO-LUMO gap), 29–42 (Spin/Ox./Charge), and 43–69 (Metal \& Ligand names).}
    \label{fig:fig_5}
\end{figure}

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.80\linewidth]{Images/Fig-Chap9C/figures/Figure6.pdf}
    \caption{Histogram plot of poorly predicted complexes (MAE > 10 kcal/mol) frequency against the type of metal, spin, and total charge of the complex.}
    \label{fig:fig_6}
\end{figure*}

To test the robustness of our models beyond the training domain, we designed a transferability dataset composed of complexes with bidentate ligands and extended $\pi$-conjugation. We refined our descriptor set (DC-T) to exclude ligand-specific features while retaining this task's critical electronic descriptors and metal identity. Despite these reductions, the MLP-T model achieved a promising transferability MAE of 9.9 kcal/mol, with nearly 50\% of predictions deviating less than 7 kcal/mol from DFT references (Figure~\ref{fig:fig_7}). This suggests that property-based descriptors capture transferrable patterns of SSE behavior, though limitations remain for outlier systems such as Fe(NCH)$_6^{2+}$. These findings highlight the potential and boundaries of our framework and motivate future work on descriptor generalization and chemically aware feature engineering.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.99\linewidth]{Images/Fig-Chap9C/figures/Figure7.pdf}
    \caption{Line plots of Actual and Predicted SSE for Transferability set.}
    \label{fig:fig_7}
\end{figure}


\section{Conclusion}

This work explores the design of descriptors grounded in electronic structure theory to enable accurate spin state energy (SSE) predictions across diverse chemical spaces. Motivated by the hypothesis that SSE gaps can be inferred from a single high-spin (HS) calculation, we demonstrate that key quantities such as d-orbital eigenvalues and natural charges obtained from HS configurations exhibit strong correlations with SSE. Moreover, incorporating experimentally accessible atomic spectra from the NIST database enhances model performance, highlighting the potential of integrating empirical data into descriptor sets.

Our best-performing model, a simple multilayer perceptron (MLP) with only two hidden layers (60,10), achieves a test MAE of 4.0 kcal/mol on monodentate complexes. Significantly, this framework extends beyond the training domain, successfully transferring predictive capabilities to a distinct class of complexes featuring bidentate $\pi$-accepting ligands. This work underscores the value of electronic structure-based and transferable descriptors for generalizable ML models in transition metal chemistry, paving the way for broader applicability in designing spin crossover materials and catalysts.

==> Chapters/chapter3.tex <==
\chapter{Fast and Efficient Inverse of Convolution Layer}\label{chap:finc}

\section{Introduction}
% \section{FInC Flow}
Since their introduction in Glow, invertible convolutions have been a fundamental component for developing expressive normalizing flow-based generative models. There have been several attempts to develop invertible $k \times k$ convolutions that are effective in training and sampling passes. In terms of sampling time, although these approaches enhanced the expressiveness and sampling efficiency, they lagged far behind Glow, which employed only $1 \times 1$ convolutions. In addition, several techniques conceal many parameters of the underlying convolution, resulting in diminished expressivity with a fixed runtime budget. We propose a $k \times k$ convolutional layer and Deep Normalizing Flow architecture that i.) has a fast parallel inversion algorithm with running time $O(H + W)$, ii.) masks the minimal amount of learnable parameters in a layer, and iii.) provides comparable forward pass and sampling times to Glow on real-world benchmarks. We implement the recommended parallel technique for sampling utilizing our GPU-based invertible convolutions; see Figure \ref{fastflow}. CIFAR, ImageNet, and CelebA benchmark datasets show comparable performance (see Figure \ref{fig:celeba_reconstruct}) to previous works in bits per dimension while significantly improving the sampling time \cite{visapp23}.


\begin{table}[!ht]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l l l l r}
        \toprule
        Method    & \# of ops & \#params/layer & Complexity of Jacobian & Inverse\\ 
        \midrule
        FInC Flow (our)  &    $(2n-1)k^2$ & $k^2 - 1$    & 1 &     exact   \\
        Woodbury \citep{lu2020woodbury} & $cn^2$ & $k^2$ & O$(d^2(c + n) + d^3)$ & exact \\
        MaCow \citep{ma2019macow}     &  $4nk^2$   & $k( \lceil \frac{k}{2} \rceil -1$) &  O$(n^3)$ & exact\\ 
        Emerging \citep{hoogeboom2019emerging}  &  $2n^2k^2$ &  $k( \lceil \frac{k}{2} \rceil -1$)  &  O$(n)$  &    exact   \\
        CInC Flow \citep{nagar2021cinc}  &  $n^2 k^2$   & $k^2 - 1$    & 1  &   exact      \\
        \midrule
        MintNet   \citep{song2019mintnet} &  $3n$   &  $ \frac{k^2}{3}$   &  O$(n)$ &    approx  \\ 
        SNF  \citep{keller2021self} &   $k^2$   &  $k^2$  &  approx &  approx \\ \bottomrule
    \end{tabular}
    } 
    \caption{Comparison of the learnable parameters. where $ n \times n $ is input size, $k \times k$ is filter size which is constant, $c$ is number of input/output channels. $d$ is the number of latent dimensions. \# of ops: required number of operations for the inversion of convolutional layers. The complexity of Jacobian: Time complexity for calculating the Jacobian of a single convolution layer. For FInC Flow and CInC Flow, the Jacobian is 1, since the Convolution matrix is lower triangular with diagonal entries being 1.}
    \label{table:complexity}
\end{table}

\section{Related Work}
\paragraph{Generative Modeling:}
The idea of generative modeling stems from training a generative model whose sample comes from the same distribution as the training data distribution. Most of the generative models can be grouped as Generative adversarial networks (GANs) \citep{goodfellow2014generative, brock2018large}, Energy-based models (EBMs) \citep{zhang2022generative, song2021maximum}, Variational autoencoders (VAEs) \citep{kingma2013auto, kingma2018variational, hazami2022efficient}, Autoregressive models \citep{oord2016wavenet, nash2020polygen}, Diffusion models \citep{ho2020denoising, song2021scorebased, song2019generative} and Flow-based models \citep{dinh2014nice, dinh2016density, hoogeboom2019emerging,kingma2018glow, ho2019flow++, ma2019macow, nagar2021cinc}. 

\paragraph{Normalizing Flows.}
Flows-based models construct complex distributions by transforming a probability density through a series of invertible mappings \citep{rezende2015variational}. At the end of these invertible mappings, we obtain a valid distribution; hence, this type of flow is referred to as a Normalizing Flow model. Flow models apply the rule for change of variables; the initial density ‘flows’ through the sequence of invertible mappings \citep{dinh2016density}. Flow-based models generalize a dataset distribution into a latent space \citep{kobyzev2020normalizing}.


\paragraph{Invertible kxk Convolutions:}
% Two types of invertible convolutions. Methods with exact inverses
An invertible neural network requires the inverse of the network with fast and efficient computation of the Jacobian determinant \citep{song2019mintnet}. An invertible neural network with more interpretability can be used for generation and classification. \citep{kingma2018glow} proposed an invertible $1 \times 1$ convolution building on top of NICE \citep{dinh2014nice}  and RealNVP \citep{dinh2016density}, consisting of a series of flow steps combined in a multi-scale architecture. Each flow step consists of an actnorm followed by an invertible $1 \times 1$ convolution, followed by a coupling layer (see Sec \ref{section:fastflowunit}). Emerging \citep{hoogeboom2019emerging} presented a method to generalize $1 \times 1$ convolution to invertible $ k \times k$ convolutions. Emerging chains two specific auto-regressive convolutions \citep{kingma2013auto} to form a single convolutional layer following the associativity of the convolution operation. Each of these autoregressive convolutions is chosen such that the resulting convolution matrix $\mathbf{M}$ is triangular, and the inverse time of each of the convolutions is O$(n  \times n \times k^2)$. MintNet \citep{song2019mintnet} presented a method for designing invertible neural networks by combining building blocks with a set of composition rules. The inversion of the proposed blocks necessitates a sequence of dependent computations that increase the network's sampling time. SNF \citep{keller2021self} proposed a method to reduce the computation complexity of the Jacobian determinant by replacing the gradient term with a learned approximate inverse for each layer. This method avoids the determinant of the Jacobian and makes it approximate, but it requires an additional backward pass for inversion of the convolution. MaCow \citep{ma2019macow} while many other papers make use of the invertibility of triangular matrix to reduce inversion time, MaCow outperforms all of them by performing the inverse in O$(n k^2)$ by carefully masking $4$ kernels at the top, left, bottom, right to achieve a full convolution, but this flow model uses four autoregressive convolutions to make an effective standard convolution. Woodbury \citep{lu2020woodbury} this paper employs the \emph{Woodbury transformation} for invertible convolution, which is a generalized permutation layer that models dimension dependencies along the channel and spatial axes using the channel and spatial transformation. ButterflyFlow \citep{meng2022butterflyflow} introduced a new family of an invertible layer that works for special underlying structures and needs a sequence of layers for an effective invertible convolution.
%  write more 


\paragraph{Fast Algorithms for Invertible Convolutions:}
CInC Flow \citep{nagar2021cinc}, derive necessary and sufficient conditions on a padded CNN for it to be invertible and require a single CNN layer for every effective invertible CNN layer. The padded CNN can leverage the advantage of parallel computation for inversion, resulting in faster and more efficient computation of Jacobian determinants.

The distinguishing feature of our invertible convolutions as compared to previous works is that we have a parallel inversion algorithm that does only $(2n-1)k^2$ operations, where $n$ is the input size and $k$ is the kernel size. MaCow is the closest approach, taking twice the number of operations. Some of the approaches, like MintNet and SNF, do achieve a lesser number of operations. However, they do not properly normalize flows as they compute only an approximate inverse. We use the convolution design from CInC Flow but provide a parallel inversion algorithm. Furthermore, our FInC Flow \emph{Unit} is designed to efficiently parallelize the operations by splitting the convolution operations channel-wise. In Table \ref{table:complexity}, we compare our proposed flow model with the existing model in terms of the receptive fields/number of learnable parameters and complexity of computing the inverse of the convolution layer for sampling.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%           TRASH
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Preliminaries}\label{sec:FastFlow}
\paragraph{Normalizing Flows.}
% Define what they are.
Formally, Normalizing Flows is a series of transformations of a known simple probability density into a much more complex probability density using invertible and differentiable functions. These invertible functions allow us to write the output probability as a differentiable function of the model parameters. As a result, the models can be trained using backpropagation with the negative log-likelihood loss function.

Let $\mathbf{X} \in \mathbb{R}^d$ be a random variable with tractable density $p_\mathbf{X}$. Let $f:\mathbb{R}^d \rightarrow \mathbb{R}^{d}$ be a differentiable and invertible function. If $\mathbf{Y} = f(\mathbf{X})$ then the density of $Y$ can be calculated as 
$$ p_X(x) = p_Y(y) \left| \det J_f  \right| \qquad \text{ where } \qquad J_f =  \frac{\partial f(x)}{\partial x}.$$ 

Note that $J_f$ is a $d \times d$ matrix called the Jacobian. If $X$ is transformed using a sequence of functions $f_i$'s. That is
$f = f_1 \circ f_2 \circ f_3 \circ \cdots \circ f_r$. Now probability density, $p_Y(y)$ can be expressed as 
\begin{equation}
    p_Y(y) = p_X(f^{-1}(y)) \cdot \displaystyle \prod_{i = r}^{1}  |J_{f_i^{-1}}(y_i)| .
\end{equation}
where $ y_i = f_i^{-1}\circ \cdots \circ f_r^{-1}(x)$.
The log-probability of $p_Y$, which will be used to model the complex image distribution, is given by,
\begin{equation}
\label{eq:nll}
    \log p_Y(y) = \log p_X(f^{-1}(y_r)) + \displaystyle \sum_{i=1}^{r}  \log |\det 
    J_{f^{-1}_i}(y_i)|.
\end{equation}
The functions $f_i^{-1}$ will be given by neural network layers, and the above function can be computed during the forward pass of the neural network. The negative of this function, called the negative log-likelihood (NLL), is minimized when images in the dataset are given the highest probabilities. Hence, it gives a simple, interpretable loss function for training the model. 

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\textwidth]{Images/Fig-Chap3/FInCFlow_model.pdf}
    \caption{(a) FInC Flow unit: to utilize the independence of convolution on channels, the input channels are sliced into four equal parts and then padded (1. top-left, 2. top-right, 3. bottom-right, 4. bottom-left) to keep the input size and output size the same. Next, parallelly convoluted each sliced channel with the corresponding masked kernel (masked corners of kernels: 1. bottom-right, 2. bottom-left, 3. top-left, 4. top-right). Finally, concatenate the output from each convolution. (b) We propose a FInC Flow architecture  \ref{section:fastflowunit} where each FInC Flow \emph{Step}  consists of an actnorm step, followed by an invertible 1 × 1 convolution, followed by a coupling layer. (c) Flow is combined with a multi-scale architecture \ref{subsec:arch}.}
    \label{fastflow}
\end{figure}

\paragraph{Invertible Convolutions.}

The convolution of an input $X$ with shape $H \times W \times C$ with a kernel $K$ with shape $k \times k \times C \times C$ is $Y = X \times K$ of shape $(H - (k+1)) \times (W -  (k+1)) \times C$ which is equal to
\begin{equation}
Y_{i,j,c_o} = \sum_{l,h < k} \sum_{c_i=1}^{C} X_{i+l,j+k,c_i}K_{l,k,c_i,c_o} 
\end{equation}
Notice that the dimensions of $X$ and $Y$ are not necessarily the same. To ensure that the $X$ and $Y$ are the same size, we apply padding to the input $X$. For an input image $X$ with shape $H \times W \times C$, the $(t,b,l,r)$ padding of $X$ is the image $\hat{X}$ of shape $(H+t+b) \times (W+l+r) \times C$ is defined as
\begin{equation}
\hat{X}_{i, j, c} = 
    \begin{cases}
        X_{i-t, j-l, c} & \text{if } i - t < H \text{ and } j - l < W \\
        0 & \text{otherwise}
    \end{cases}
\end{equation}
The convolution operation is a linear transformation of the input. For the vector (flattened) input $X$, denoted by $x$, the output vector $y$ can be written as  $y = \mathbf{M} x$. Matrix $\mathbf{M}$ is called the \emph{Convolution Matrix}, and the dimensions of this matrix are $HWC \times HWC$. As long as the matrix $\mathbf{M}$ is invertible, the convolutional layer can be included as a part of the Normalizing Flows. The common approach to building invertible convolutions is to make $M$ upper triangular and ensure invertibility by making the diagonal entries nonzero.



\paragraph{Algorithms for Computing Inverse of Convolutions.}
For normalizing flows built using invertible convolutions, the sampling pass will involve computing the inverse of the convolution matrix. This involves solving a linear system of equations $\textbf{M}x =y$.

For a general square matrix of size $n \times n$, the time complexity for inversion is $O( n^3)$. For a lower triangular matrix of size $n \times n$, the time complexity for inversion is $O(n^2)$ because of the back-substitution method. Notice that the size of the convolution matrix, \textbf{M}) is $n^2 \times n^2$ (refer Figure \ref{fig:Conv_equn}) and also that row of the matrix has only $k^2$ entries at the maximum, resulting in an inversion time of $O(n^{2} k^{2})$ which is used in many of the previous works like Emerging and CInC Flows. We show that this method can be parallelized for carefully designed convolutions, giving a complexity of only $O(n k^2)$.

\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{Images/Fig-Chap3/Conv_equn.pdf}
    \caption{Linear transformation of invertible convolution, $n = 2$, $K = 2$ with $K-1$ top and left padding.}
    \label{fig:Conv_equn}
\end{figure}


\section{FInC Flow: Our Approach}
In this section, we describe our approach, including a convolution layer design with a fast parallel inversion algorithm with running time O$(n k^2)$. For more clarity, we refer to the height of the image as $H$, the width as $W$, and the channels as $C$ in this section.


\paragraph{Convolution Design} \label{sec:conv-design}
As it is obvious from equation $ x = \textbf{M}^{-1} y$, the inverse timings depend on $\mathbf{M}$. Emerging \citep{behrmann2019invertible} masks almost half of the convolution kernel values to ensure $\textbf{M}$ is a Lower Triangular Matrix. However, we follow the method followed in CInC Flow, where only a few values of the convolution kernel are masked.
% \noindent
For an input image $X$ with shape $H \times W \times C$, the top-left(\emph{TL}) i.e., $(t, 0, l, 0)$ padding of $X$ is the image $X^{\text{(TL)}}$ of shape $(H+t) \times (W+l) \times C$ is defined in equation \ref{eq:top_left_padding} and similarly for the top-right (\emph{TR}) as equation \ref{eq:top_right_padding}, bottom-left (\emph{BL}) as equation \ref{eq:bottom_left_padding}, bottom-right (\emph{BR}) as equation \ref{eq:bottom_right_padding}. 
\begin{align}
    X^{\text{(TL)}}_{i, j, c} &= 
    \begin{cases}
        X_{i-t, j-l, c} & i - t > 0 ~\wedge~ 
        j - l > 0 \\
        0 &\text{otherwise}
    \end{cases} \label{eq:top_left_padding} \\
    X^{\text{(TR)}}_{i, j, c} &= 
    \begin{cases}
        X_{i-t, j, c}~~~ &  i - t > 0 ~\wedge~ j - r < W \\
        0 &\text{otherwise}
    \end{cases} \label{eq:top_right_padding} \\
    X^{\text{(BL)}}_{i, j, c} &= 
    \begin{cases}
        X_{i, j-l, c}~~~~ &  i - b < H ~\wedge~ j - l > 0 \\
        0 &\text{otherwise}
    \end{cases} \label{eq:bottom_left_padding}\\
    X^{\text{(BR)}}_{i, j, c} &= 
    \begin{cases}
        X_{i, j, c}~~~~~~~~ &  i - b < H ~\wedge~ j - r < W \\
        0 &\text{otherwise}
    \end{cases}  \label{eq:bottom_right_padding}
\end{align}
Figure \ref{fig:Conv_equn} shows that the convolution of a \emph{TL} padded $3 \times 3$ image with a $2 \times 2$ filter is equivalent to a matrix multiplication between the convolution matrix $\textbf{M}$ and the vector input $x$.  We leverage this to find the inverse faster. We discuss this in more detail in the subsequent sections. Also padded input $X^{\text{(TR)}}$, $X^{\text{(BL)}}$ and $X^{\text{(BR)}}$ are equivalent to $X^{\text{(TL)}}$ once they are flipped along corresponding dimension(s).  


\SetKwComment{Comment}{/* }{ */}

\begin{algorithm}[!ht] 
    \caption{Fast Parallel Inversion Algorithm of \emph{TL} padded convolution block(PCB)}
    \label{alg:inv_algo}
    \KwIn{$K$: Kernel of shape $(C, C, k_H, k_W)$\\
    $Y$: output of the conv of shape $(C, H, W)$}
    \KwResult{$X$: inverse of the conv. with shape $(C, H, W)$.}
    \textbf{Initialization:} $X \gets Y$ \;
    \For{$d \gets 0, H + W - 1$}{
        \For {$ c \gets 0, C - 1 $}{
            \Comment{The below lines of code execute in parallel on different threads on the GPU for every index $(c, h, w)$ of $X$  on the $d$th diagonal.} 
            
                \For{$ k_h \gets 0, k_H - 1 $}{
                \For{$ k_w \gets 0, k_W - 1 $}{
                \For{$ k_c \gets 0, C - 1 $}{
                    \If{pixel $ (k_c, h - k_h, w - k_w) $ not out of bounds}{
                         $ X[c, h, w]  \gets X[c, h, w] - X[k_c,h - k_h, w - k_w] * K[c, k_c, k_H - k_h - 1, k_W - k_w - 1]; $
                      }
                }
                }
                } \Comment{synchronize all threads}
        } 
     }
\end{algorithm}

\paragraph{Parallel Inversion Algorithm}\label{subsec:PIA}
We have presented our algorithm in Algorithm \ref{alg:inv_algo}. The algorithm can be understood using Figure \ref{fig:Conv_equn}. 


\begin{definition}[Diagonal Elements]
Two pixels $x_{i, j}$ and $x_{i', j'}$ are said to be secondary diagonal elements if $i + i' = j+j'$ . For brevity, we refer to these elements from here on simply as Diagonal Elements.
\end{definition}


Theorem \ref{th:ind_parallel} proves that every element on the diagonal can be computed in parallel, and Line 2 of the algorithm takes care of that. We initialize $X$ to $Y$ in Line 1 and compute $X$ in Line 8, which is given in Equation \ref{eq:inv_convolution_imp}. 
It is important that we wait for the threads to synchronize before we move to the next diagonal, as they are needed for computing the elements of the next diagonal. The \emph{not out of bounds} in Line 7 means we are remaining in the $k \times k$ convolution window and also we are not including pixel $(i, j)$ while computing $x_{i, j}$ as given in Equation \ref{eq:inv_convolution_imp}


\begin{theorem}
\label{th:ind_parallel}
The inverse of the pixels on the diagonals of a TL-padded convolution can be computed independently and in parallel.
\end{theorem}
% \renewcommand\qedsymbol{QED}
\begin{proof}
The $(i, j)^{th}$ pixel value of the output $Y$ with shape $H \times W$ can be calculated as 
$$
y_{i, j} = (\textbf{M}_{iW+j, :})^T \cdot x
$$ 
which means $y_{i,j}$ is the dot product of $\textbf{M}_{iW+j, :}$ i.e., the corresponding row of matrix $\textbf{M}$ and the vectored input $x$.
Because it is a \emph{TL} padded convolution, $y_{i,j}$ depends only on the values of $k \times k$ window of $x_{\le i, \le j}$ pixels where $x_{\le i, \le j}$ are the pixels that are on the top and left side of the pixel $x_{i, j}$ including $x_{i, j}$. Because all the diagonal values are $w_{k, k}$, we have, 
\begin{align*}
y_{i, j} &= w_{k, k} x_{i, j} + f(x_{<i, <j})\\ 
x_{i, j} &= \frac{y_{i, j} - f(x_{<i, <j})}{w_{k, k}}   
\end{align*}

where $x_{<i, <j}$ are the pixels that are strictly on top and left side of $(i, j)$. Following the masking pattern of CInC Flow, we have $w_{k, k} = 1$, and $f$ is a linear function that is given by the weighted sum of the given pixels, weighed by the filter values. So,
\begin{equation}
\label{eq:inv_convolution}
x_{i, j} = y_{i, j} - f(x_{<i, <j})
\end{equation}
\begin{equation}
\label{eq:inv_convolution_imp}
x_{i, j} = y_{i, j} - \sum_{p=0}^{k} \sum_{q=0}^{k} x_{i-p, j-q} K_{p, q}  \text{ where }  p = q \neq 0
\end{equation}

% \noindent
Let two pixels $x_{i, j}$ and $x_{i', j'}$ be on the same diagonal. This also means that only one of the following settings is true a) $i < i'$ and $j > j'$ or b) $i > i'$ or $j < j'$. Either way, we can conclude that the computation of $x_{i, j}$ is not dependent on $x_{i', j'}$ and vice versa, following the result in Equation \ref{eq:inv_convolution}. Hence, they can be computed independently.
% \noindent
Once $x_{i, j}$ is computed, following the Equation \ref{eq:inv_convolution} and the above result, we can compute $x_{i + 1, j}$ and $x_{i, j+1}$. Since, the sets of pixels $x_{<i+1, <j}$ and $x_{<i, <j+1}$ both include the elements of $x_{<i, j}$ and also $x_{i, j}$, we can write
\begin{align}
x_{i + 1, j} &= y_{i+1, j} - f(x_{<i+1, <j}) \nonumber\\
&=y_{i+1, j} - \alpha x_{i, j} - f_1(x_{<i, <j})\label{eq:parallel_1}\\
x_{i, j+1} &= y_{i, j+1} - f(x_{<i, <j+1}) \nonumber\\
&=y_{i, j+1} - \beta x_{i, j} - f_2(x_{<i, <j}) \label{eq:parallel_2}
\end{align}

where $\alpha$ and $\beta$ are kernel weights.

From Equations \ref{eq:parallel_1}  and \ref{eq:parallel_2}, we can conclude that $x_{i+1, j}$ and $x_{i, j+1}$, which are on the same diagonal, can be calculated in parallel in a single step.
\end{proof}

\begin{theorem}
Algorithm \ref{alg:inv_algo} uses only $(H+W-1)k^2$ sequential operations.
\end{theorem}

\begin{proof}
We have proved in Theorem \ref{th:ind_parallel} that the inverse pixels on a single diagonal can be computed in parallel in one iteration of Algorithm \ref{alg:inv_algo}. Since there are $H + W - 1$ diagonals in a matrix and there are at most $k^2$ entries in a row of the convolutional matrix, the number of sequential operations needed will be $(H+W-1)k^2$.
\end{proof}

Thus the running time of our algorithm is O$(n k^2)$ where $n = H = W$ 

\begin{table}[!ht]

    \centering
       \resizebox{\textwidth}{!}{% <------ Don't forget this %
    \begin{tabular}{lcccccccccccc}
        \toprule
        \multicolumn{1}{l}{Model} & \multicolumn{3}{c}{MNIST} & \multicolumn{3}{c}{CIFAR-10} & \multicolumn{3}{c}{Imagenet-32x32} & \multicolumn{3}{c}{Imagenet-64x64}\\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
           &   BPD &  FT & ST &  BPD &  FT & ST & BPD &  FT  &  ST   &   BPD  & FT & ST\\
        \midrule
        % Glow    &   1.05 &  0.14 & 0.08 &  3.36 & 0.40 & 0.22 & 4.12 & 0.59 & 0.37   &   3.81  & 1.51 & 1.17\\
        % Flow++ \citep{ho2019flow++} &   -- &  -- & -- &  3.08 & 1.35 & 1.71 &  3.86 &    2.75  &     2.49   &   3.69  &  16.47 &  1.89\\
        % SNF &  1.06 &  0.09 & 0.09 &  3.37 & 0.23 & 0.21 &  4.14 &    0.34  &     0.31   &    --  &  1.17 &  1.13\\
        % \hline
        Emerging &   -- &  0.16 & 0.62 &  3.34 & 0.49 & 17.19 &  4.09 &    0.73  &    25.79   &    3.81  &  1.71 &  137.04\\
        MaCow   &   -- &  --& -- &  3.16 & 1.49 & 3.23 &  -- &    --  &     --   &    3.69  &  2.91 &  8.05\\
        % Woodbury &   -- &  --& -- &  3.47 & -- & -- &  4.20 &    --  &     --   &    3.87  &  -- &  --\\
        CInC Flow & -- &  --& -- &  3.35 & 0.42 & 7.91 &  4.03 &   0.62  &     11.97   &    3.85  &  1.57 &  55.71\\
        MintNet & 0.98 &  0.16 & 17.29 &  3.32 & 2.09 & 230.17 &  4.06 &    2.08  &     230.44   &    --  &  -- &  --\\
        %WaveFlow & -- &  -- & -- &  -- & -- & -- &  4.08 &    --  &     --   &    3.78  &  -- &  --   \\%
        FInC Flow (our) &   1.05 &  0.14 & 0.09 &  3.39 & 0.37 & 0.41 &  4.13 &    0.48  &  0.52   &    3.88  &  1.43 & 2.11 \\  
        \bottomrule
        \end{tabular}
        }%
    \caption{Comparison of the bits per dimension (BPD), forward pass time (FT), and sampling time (ST) on standard benchmark datasets of various $k \times k$ convolution-based Normalizing Flow models. FT and ST are presented in seconds.}
    \label{table:bpd_table}
\end{table}

\paragraph{FInC Flow Unit}\label{section:fastflowunit}

Figure \ref{fastflow} visualizes our $ \ k\times k$ convolution block. We call this block as FInC Flow \emph{Unit}. We use all the $4$ padding techniques mentioned before for different channels of the image. For this purpose, we split the input into four equal parts along the channel axis. We do \emph{TL} padding to the first part, \emph{TR} to the second part, \emph{BL} to the third part, and \emph{BR} to the fourth part. Then, we use a masked filter on each of these parts to perform the convolution operation in parallel. We call each of these padded images, along with its corresponding kernel, a Padded Convolution Block (PCB).


\paragraph{Architecture}\label{subsec:arch}
Figure \ref{fastflow}c shows the complete architecture of our model. Our model architecture resembles the architecture of Glow. The multi-scale architecture involves a block of a Squeeze layer, FInC Flow \emph{Step} repeated $K$ a number of times, and a Split layer. The whole block is repeated $L - 1$ a number of times. A Squeeze layer follows this, and finally, FInC Flow \emph{Step} repeated $K$ times.
Half of the channels are 'split' (taken away) at the end of each split layer and modeled as Gaussian distribution samples. These split-half channels are \emph{latent vectors}. The same is done for the output channels. These are denoted as $z_L$ in Figure \ref{fastflow}(c). 
Each \emph{FInC Flow Step} consists of a \emph{FInC Flow Unit}, an Actnorm Layer, a $1 \times 1$ Convolutional Layer, followed by a coupling layer. \\
\textbf{Actnorm Layer:} Acts as an activation normalization layer similar to that of a batch normalization layer. Introduced in Glow, this layer performs the affine transformation using scale and bias parameters per channel. 
\\
\textbf{$1 \times 1$ Convolutional Layer:} This layer introduced in Glow does a $1 \times 1$ convolution for a given input. Its log determinant and inverse are very easy to compute. It also improves the effectiveness of coupling layers.
\\
\textbf{Coupling Layer:} RealNVP introduced a layer in which the input is split into two halves. The first half remains unchanged, and the second half is transformed and parameterized by the first half. The output is the concatenation of the first half and the affine transformation by functions parameterized by the first half of the second half. The inverse and log determinants of the coupling layer are computed in a straightforward manner. The coupling layer consists of a $3 \times 3$ convolution followed by a $1 \times 1$ and a modified $3 \times 3$ convolution used in Emerging.
\\
\textbf{Squeeze:} This layer takes features from the spatial to the channel dimension \citep{behrmann2019invertible}, i.e., it reduces the feature dimension by a total of four, two across the height dimension and two across the width dimension, resulting in an increase in the channel dimension by four. As used by \citep{dinh2016density}, we use a squeeze layer to reshape the feature maps to have smaller resolutions but more channels.
\\
\textbf{Split:} Input is split into two halves across the channel dimension. We retain the first half, and a function parameterized by the first half transforms the second half. The transformed second half is modeled as Gaussian samples of the \emph{latent vectors}. We do not use the checkerboard pattern used in RealNVP \citep{dinh2016density} and many others to keep the architecture simple.

\SetKwComment{Comment}{/* }{ */}


\begin{figure}
    % \vspace{-02em}
    \centering
    \includegraphics[width=0.79\linewidth]{Images/Fig-Chap3/diag_and_conv_matrix.pdf}
    \caption{ (a) Convolution Matrix $M$ obtained for a $4 \times 4 \times 2$ image with a $2 \times 2 \times 2 \times 2$ filter. (b) Parallel Computation in a $6 \times 6$ Image. Pixels with the same color have their inverses calculated in parallel.}
    % \vspace{-2em}
    \label{fig:conv_parallel}
\end{figure}


\begin{table}[!ht]
    \centering
    \resizebox{\textwidth}{!}{% <------ Don't forget this %
        \begin{tabular}{l  c  c  c c}
        \toprule
            Models    & Setting (K and L) & Param (M) & FT & ST \\ 
            \midrule
            MaCow-FG & [4, [12, 12], [12, 12], 12]  &  37.19M   & 0.88  & 2.64  \\
            MaCow-org &  [4, [12, 12], [12, 12], 12], [4, 4]  & 38.4M & 1.48  & 3.23 \\ 
            % Glow  & [32, 32, 32]  &   44.7M  & 0.40  & 0.22    \\
            FInC Flow (our) &  [28, 28, 28] & 39.46M  & \textbf{0.37}  & \textbf{0.41}   \\
            \bottomrule
        \end{tabular}
    }
    \caption{CIFAR-10: comparison of learnable parameters and the sampling time. FInC Flow has fewer learnable parameters with the same receptive field and fast layers (all the times are averaged over ten loops for n = 100 sample images in seconds). ST = Sample time, FT = Forward Time. MaCow-FG is the fine-grained MaCow model, and MaCow-org stands for the MaCow model and utilizes the original multi-scale architecture, the same as Glow. MaCow and our method are closely similar in terms of the convolutional design. So, here we show that our proposed method does fast sampling while maintaining the faster forward time .}
    \label{table:params}
\end{table}
% \vspace{2em}

\section{Results}\label{sec:results}
% \paragraph{Negative log-likelihood / bits per dimension (BPD):}
\paragraph{Bits Per Dimension (BPD):}
BPD is closely related to NLLLoss given in equation \ref{eq:nll}. BPD of $H \times W \times C$ image is given by
\begin{equation}
\label{eq:bpd}
    \text{bpd} = \frac{\text{NLLLoss} \times\log_2{e}}{H W C} 
\end{equation}
% \noindent
Table \ref{table:bpd_table} shows the BPD comparative results of various models with our model. We present the results of MaCow-var, which uses Variational De-quantization, which was introduced in Flow++ \citep{ho2019flow++}. The recorded BPDs are the reported numbers from the respective model papers.

\paragraph{Sampling Time:}\label{section:SamplingTimes}
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.99\linewidth]{Images/Fig-Chap3/timings_95.pdf}
    \caption{Sampling Times for four models - our, Emerging, CInC Flow,  MaCow. Each plot gives the $95\%$ Confidence Interval (CI) time of the ten runs to sample $100$ images. The X-axis represents the sizes of the image sampled, starting from $16 \times 16 \times 2$ ($H \times W \times C$) all the way to $128 \times 128 \times 2$. }
    \label{fig:timing}
\end{figure*}

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.99\linewidth]{Images/Fig-Chap3/celeba_reconstruct.pdf}
    \caption{Comparison of  (a) original and (b) reconstructed image samples for the $64 \times 64$ CelebA dataset after FInC Flow model for $100$ epochs. We can conclude that our model reconstructs the original image from the images.}
    \label{fig:celeba_reconstruct}
\end{figure*}
% \vspace{8em}
Table \ref{table:bpd_table} shows the comparative results of our model with other models. For MaCow, we use the official code released by the authors. We use the code for Emerging, which was implemented in PyTorch by the authors of SNF.. We have implemented CInC Flow in PyTorch and used it to generate results.
% We have implemented Emerging \citep{hoogeboom2019emerging} and CInC Flow \citep{nagar2021cinc} in PyTorch for the same. 
The FTs and STs are recorded by averaging ten runs on untrained models (including ours). 

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.99\linewidth]{Images/Fig-Chap3/uncurated_samples.pdf}
    \caption{Uncurated generated samples images from our flow model.}
    \label{fig:uncurated_samples}
\end{figure}

In Figure \ref{fig:timing}, we plot the relationship between the input image size and inverse sampling time. As the input image size increases, our \emph{Parallel Inversion Algorithm} improves by utilizing the independence in the convolution matrix $M$. If we input a single image (batch size = $1$), our model performs similarly to the CInC Flow and Emerging. MaCow is far slower because it does the masking of four kernels to maintain the receptive field. To do one convolution, four convolutions are needed to complete one standard convolution, making it slower. Emerging requires two consecutive autoregressive convolutions to have the same receptive field as standard convolution and solver, compared to FInC Flow. For batch size = $4$ and larger, FInC Flow beats the Emerging, MaCow, and CInC Flow by a big difference (see Figure \ref{fig:timing}) while maintaining the same receptive field. 


\paragraph{Scaling sampling time with spatial dimensions:}
Table \ref{table:params} shows the comparison among the invertible convolution-based models. To keep it fair, we restrict the total parameters across all the models to be close to $5$ M. We note down the average sampling time (ST) to generate $100$ images over ten runs while doubling the size of the sampled image from $16 \times 16$ all the way to $128 \times 128$ and also doubling our batch size from $1$ all the way to $128$. Our model outperforms all the other models in most, if not all, settings. All the models were untrained and ran on a single NVIDIA GTX 1080 Ti GPU.
\paragraph{Image reconstruction and generation:}
In Figure \ref{fig:celeba_reconstruct}, we present the effectiveness of the  FInC Flow model in the reconstruction (sampling) of the images. First, we feed the input image to the forward flow and get the \emph{latent vector} ($z_L$). To reconstruct the images from the \emph{latent vector} ($z_L$), give the $z$ as input to the inverse flow. Figure \ref{fig:celeba_reconstruct} presents the reconstructed face images for the CelebA dataset after training our model for $100$ epochs. The model takes a random sample from the Gaussian distribution for the \emph{latent vector} to generate sample images. This \emph{latent vector} is used to generate images by going backward in the flow model. In Figure \ref{fig:uncurated_samples}, we present a generated sample by our model on the MNIST, CIFAR-10, and ImageNet-64x64 datasets.

\section{Summary}
We present a $k\times k$ invertible convolution with a parallel inversion algorithm. We use it to build a normalizing flow architecture that is highly efficient in the sampling pass. We implemented our parallel algorithm on a GPU and presented benchmarking results, which show significant improvement in sampling times and forward time compared to other  $  k\times k$ invertible convolution approaches. The Normalizing flow's problem is the slow inversion of the convolution layers. This work presents a fast and invertible convolutional layer for padded input. Our proposed FInC Flow models show consistent improvements over various datasets using the same parameter budget, making the inversion faster when considering models constrained in a bigger batch size and input image size. FInC Flow maintains significant sampling time differences with existing flow models such as Emerging, MaCow, Woodbury, and SNF. The generated samples show an unprecedented amount of semantic coherence and exactness of details even at the small scale size of full 8-bit $64 \times 64$ images.

\section*{Additional details}
Code for our implementation is available here:   \\\url{https://github.com/aditya-v-kallappa/FInCFlow}
\noindent
\paragraph{Datasets}
% with citations
We train our model on standard benchmark datasets MNIST \citep{deng2012mnist}, CIFAR-10 \citep{krizhevsky2009learning}, and ImageNet \citep{russakovsky2015imagenet} sampled down to $32 \times 32$ and $64 \times 64$. We also train our model on CelebA \citep{liu2015deep} sampled down to $64 \times 64$. Figure \ref{fig:celeba_reconstruct}a presents the CelebA-$64 \times 64$ reconstructed samples, and Figure \ref{fig:uncurated_samples}b presents the CIFAR-10 and ImageNet-64x64 generated samples.

\paragraph{Hyperparameters}
To train our model, we use Adam optimizer \citep{kingma2014adam} with a learning rate of 0.001 with an exponential decay of 0.99997 per epoch. For training on Imagenet, we also make sure that the gradients stay between $ -1$ and $ +1$ by clipping them. 

\paragraph{Masking}
To make sure the masked values in the Padded Conv Blocks, we ensure they are not affected by backpropagation. To achieve this, we reset the gradients of the masked values to zero after every training iteration.

\paragraph{Cuda code details}
To run CUDA code, we use PyTorch-LTS 1.8.2 and cudatoolkit 10.2. While we can implement Algorithm \ref{alg:finc_flow_inverse} to find the inverse of each padded block individually, we can take advantage of the fact that all 4 Padded Conv Blocks are equivalent after proper flipping of padded inputs and kernels. This is done by using Algorithm \ref{alg:finc_flow_inverse} on a GPU.

\noindent
First, we split $Y$ into 4 parts across channel dimensions following the architecture shown in 2. This is given in Line 1. Then, we flip $Y$ and kernels to match TL-padding, which is given in Line 2. Then, we concatenate them to get the final $Y$ and $K$, respectively, which are given in Lines 3 and 4. Then we apply Algorithm \ref{alg:finc_flow_inverse} to find the inverse. We do the reverse process of the above to get the correct $X$. The steps are given in Lines 5, 6, 7, and 8.

\noindent
We fix the number of threads of each grid of the GPU to be 1024, the number of $grids_x$ to be the batch size, and $grids_y$ to be 4, which is the number of Padded Conv Blocks in a single FInC Flow Unit. This ensures that not only does the GPU invert the whole FInC Flow Unit at once, but also on a batch of images. 

\begin{algorithm}[!ht]
    \caption{Fast Parallel Inversion Algorithm for FInC Flow \emph{Unit}}
    \label{alg:finc_flow_inverse}
    \KwIn{$K_1, K_2, K_3, K_4$ - Convolution Kernels of different PCB, $Y$ -  Output of the FInC Flow \emph{Unit}}
    \KwResult{$X$-Input to the FInC Flow Unit / Inverse of the FInC Flow Unit}
    \begin{enumerate}
        \item{$Y_1, Y_2, Y_3, Y_4 \gets split(Y)$ }
        \item{Flip $Y_2, Y_3, Y_4, K_2, K_3, K_4$ (in-place) appropriately to match \emph{TL} padding}
        \item{$X \gets concat(Y_1, Y_2, Y_3, Y_4)$}
        \item{$K \gets concat(K_1, K_2, K_3, K_4)$}
        \item{Apply Algorithm \ref{alg:inv_algo} with input $K, Y$  to get $X$}
        \item{$X_1, X_2, X_3, X_4 \gets split(X)$}
        \item{Flip $X_2, X_3, X_4$ appropriately to get the correct output }
        \item{$X \gets concat(X_1, X_2, X_3, X_4$)}
    \end{enumerate}
\end{algorithm}


\paragraph{Running MaCow, Emerging, CInC Flow, SNF}
For MaCow and SNF, we use the official code released by the authors. Emerging was implemented in PyTorch by the authors of SNF. We make use of that. We have implemented CInC Flow on PyTorch to get the results.

\paragraph{Computing Run-time and Confidence Intervals}
We run the model (both forward and sampling) $11$ times and ignore the $1^{\text{st}}$ run as it includes the initialization time. We calculate the mean, standard deviation, and $95\%$ confidence interval and plot the numbers.
\\
To calculate forward time, we pass $100$ images, as for sampling times, we sample $100$ images. We present these numbers in Table-\ref{table:params}.
\\
For sampling time comparison of different models shown in Figure \ref{fig:timing}, we set the total number of parameters for all the models to be close to $5\mathbf{M}$ to make it a fair comparison. 

\paragraph{Hardware/Training Time}
Our hardware setup consists of an Intel Xeon E5-2640 v4 processor providing 40 cores, 80 GB of DDR4 RAM, and 4 Nvidia GeForce GTX 1080 Ti GPUs, each with $12$ GB of VRAM. We train our model on all GPUs using PyTorch's Data Parallel class. We implement an early stopping mechanism for smaller datasets like MNIST and CIFAR-10. For others, we train the model for a maximum of epochs. To evaluate Forward Time and Sampling Time, we use only one of the GPUs.We evaluate our FInC Flow model on MNIST, CIFAR-10, Imagenet-32x32, and Imagenet-64x64 datasets for three metrics - (a) Loss expressed in Bits per Dimension (BPD), (b) Forward Pass Time (FT): Time taken for 100 images to be passed through the model and (c) Sampling Time(ST): Time taken by the model to generate 100 images.  To do this, we train our model with Adam Optimizer with a learning rate ($lr$) of $0.001$ and exponentially reduce the $lr$ by $0.99997$ after each epoch. We have used 4 NVIDIA GTX 1080 Ti GPUs to train our model. Evaluation(FT/ST) is done on a single GPU.





==> Chapters/trash.tex <==
% \paragraph{Flow Models and Generative Models in Image Synthesis:}
% \paragraph{Mode Collapse and Lack of Diversity}
% \paragraph{Evaluation Metrics and Benchmarks}

% Evaluating the performance of normalizing flow models is another challenge, as traditional metrics like log-likelihood might not always capture the full performance of the model, especially in generative tasks. Developing robust, standardized evaluation protocols and benchmarks for normalizing flows is essential for advancing the field and consistently comparing models.
% In some cases, normalizing flow models can suffer from mode collapse, where the model learns to focus on a limited set of modes in the target distribution and fails to capture the full diversity of the data. This problem is particularly prominent in high-dimensional spaces, where the model may fail to adequately cover all input space regions. Techniques to mitigate mode collapse include regularization strategies and improved architectures such as \textit{autoregressive flows}.
% \paragraph{Choosing the Right Base Distribution}

% The choice of base distribution, often a simple distribution like a Gaussian, significantly impacts the flow model's expressiveness and learning efficiency. In practice, selecting a suitable base distribution that can adequately represent the underlying structure of the target distribution is non-trivial. A poor choice may lead to slow convergence or an inability to model the target distribution effectively.
% \paragraph{Model Selection and Hyperparameter Tuning}

% Like many machine learning models, normalizing flows require careful selection of hyperparameters, such as the number of flow steps, the architecture of the transformation functions, and the base distribution. Finding the optimal configuration often involves extensive experimentation, and the performance can be sensitive to these choices. Automated hyperparameter search methods like Bayesian optimization can help, but the tuning process remains a significant bottleneck for practitioners.
% Normalizing flows (NF) represent an essential subset within deep generative models, offering unique advantages compared to other models like Generative Adversarial Networks (GANs) and Variational Autoencoders (VAEs). Unlike GANs and VAEs, which involve adversarial or variational training techniques, normalizing flows utilize a straightforward maximum likelihood loss function for training. In flow models, each image corresponds directly to a latent vector following a Gaussian distribution, establishing a one-to-one mapping that aids interpretability and control in image generation tasks. However, despite these benefits, GANs and VAEs are often preferred due to the practical limitations of flow-based models. The primary challenge lies in the requirement for invertibility within NFs transformations, which restricts the choice of neural network architectures and necessitates efficient computation of these transformations in both forward and sampling stages.

% An essential advancement in normalizing flow-based generative models came with the introduction of Glow \cite{glow}, which utilized $1 \times 1$ invertible convolutions. The significant advantage of $1 \times 1$ convolutions lies in their computational efficiency: their inverse operation is also a $1 \times 1$ convolution, and they enable fast parallel computations that are invariant to spatial dimensions, making them effective in both encoding (latent vector generation) and decoding (image synthesis) processes. Although Glow paved the way for efficient normalizing flow models, \cite{glow_nxn} extending it to handle more expressive $  k\times k$ convolutions has the potential to significantly enhance its capacity for modeling complex datasets. However, this extension presents challenges as the inverse function for $k \times k$ convolutions generally requires an $n \times n$ matrix computation, resulting in costly operations during the sampling process.

% Various strategies have been proposed to overcome these limitations. Emerging Flows introduced autoregressive convolutions to approximate $n \times n$ but required two convolutions per transformation. In contrast, our work CInC Flow \cite{nagar2021cinc} employed a padded $3 \times 3$ convolution layer, optimizing parameter utilization to enhance invertibility. Despite these innovations, achieving efficient sampling and high expressivity remains an open challenge in flow-based generative modeling. Our proposed method introduces a novel flow step leveraging channel independence within convolution matrices, enabling parallel computation to accelerate sampling time without compromising model complexity.

% \paragraph{Generative Modeling Approaches}

% Generative modeling aims to train a model capable of generating samples resembling the data distribution. Major generative modeling frameworks include GANs, Energy-Based Models (EBMs), VAEs, autoregressive, and flow-based models. Flow models, in particular, hold promise for their interpretable structure and use of invertible transformations. To achieve fast invertibility, approaches like Glow, which builds on NICE and RealNVP architectures, introduced a sequence of flow steps combining actnorm, $1 \times 1$ invertible convolutions, and coupling layers in a multi-scale design. Extensions like Emerging Flows generalized these $1 \times 1$ convolutions to $d \times d$ dimensions, chaining autoregressive convolutions in layers to reduce inversion complexity. Innovations like SNF \cite{keller2021self} and MaCow further improved computational efficiency by exploiting the structure of triangular matrices. At the same time, Woodbury Flows leveraged transformation matrices along channel and spatial axes for enhanced invertibility. To address difficulties arising from low-dimensional manifolds, these models perturb data with Gaussian noise at multiple levels, iteratively estimating gradient fields for each level. This allows smooth sampling transitions from high-noise initializations to low-noise approximations, capturing intricate data characteristics without adversarial training requirements. We propose CInC Flow and Inverse Flow to achieve competitive generative performance with state-of-the-art results on CIFAR-10 and comparable outputs to GANs on MNIST, CelebA, and CIFAR-10. This framework demonstrates its robustness in applications like image deblurring and deconvolution, highlighting its potential for versatile image-based tasks.

% \paragraph{Application in Quality Assessment of Agricultural Produce:}
% Quality assessment in agriculture, particularly in seeds like corn, is a critical but often labor-intensive task. We propose a computer vision-based (generative model) system to automate this process, addressing dataset limitations through the application of a Conditional Generative Adversarial Network (CGAN) \cite{brock2018large} for synthetic image generation in underrepresented classes. Benchmarking with various image classification models on this generated dataset, we achieve high accuracy, suggesting that generative models, combined with active learning, offer a scalable solution for automated agricultural quality assessments.

% \paragraph{Generative Models and Preserving Privacy in Indian Driving Dataset:}
% As data collection for autonomous driving grows, so does the need for privacy preservation, especially with regulations like GDPR and CCPA demanding protections for personal information in public road data. Commercial solutions such as Brighter AI and Celantur offer de-identification tools, yet the lack of open datasets for face and license plate anonymization limits research advancements. This paper will introduce Pvt-IDD, the first publicly available dataset annotated for faces and license plates in real-world autonomous driving scenarios. Our work provides essential benchmarks and a baseline model to advance privacy-preserving techniques, addressing this critical gap in autonomous driving research.

% \paragraph{Stacked autoencoders and dimensionality reduction}

% In \cite{NAGAR20244502}, we present an unsupervised machine-learning framework that combines stacked autoencoders for dimensionality reduction with k-means clustering to map geological units, aiding in identifying potentially mineralized areas. The role of the stacked autoencoders is to compress data with a wide range of spectral and spatial features, enhancing the accuracy and efficiency of geological mapping. Further, our framework uses k-means clustering to generate clustered maps from the reduced dimensions. We evaluate our framework across multiple multispectral remote sensing datasets (Landsat 8, ASTER, and Sentinel-2) to map geological units in the Mutawintji region of Western New South Wales (NSW), Australia. We also compare our results with PCA and canonical autoencoders and provide open-source code to extend the study further. 


% \paragraph{Generative Models and Art Restoration:}

% Traditional supervised learning approaches hinge upon extensive collections of distorted/clean image pairs, while zero-shot methods predominantly rely on known degradation modes. However, these methodologies encounter limitations in real-world scenarios characterized by diverse and unknown distortions. To address this concern, some researchers have extended diffusion models to accommodate blind/real-world image restoration scenarios by integrating real-world distortion simulations and kernel-based techniques. This expansion seeks to bridge the gap between diffusion models and the complexity of real-world image restoration challenges, offering a potential avenue for more effective applications in practical settings.

% \par

% Normalizing flow is an essential category of Deep Generative Models that utilizes a maximum likelihood loss function, allowing for a one-to-one correspondence between images and their latent vectors, typically required to follow a Gaussian distribution. Despite their advantages over Generative Adversarial Networks (GANs) and Variational Autoencoders (VAEs), normalizing flows are less commonly used due to the necessity of invertible transformations, which limit the types of neural networks that can be employed. Key advancements in the field, such as introducing $1 \times 1$ invertible convolutions in the Glow model, have improved sampling efficiency and expressivity. However, extending these concepts to $k \times k$ convolutions presents challenges in computational efficiency during sampling, as the inverse operations can be significantly more complex. Various methods have been proposed to create efficient invertible convolutions, including autoregressive approaches and approximations for the Jacobian determinant, leading to enhanced performance in generative modeling tasks. We aim to propose a fast, efficient inverse of convolution and backpropagation algorithm and various flow models (CInc Flow, FInc Flow, Inverse Flow).



% \section{Normalizing Flow}

% Normalizing flow is a crucial subcategory of Deep Generative Models that offers distinctive benefits (\cite{kobyzev2020normalizing}). In comparison to GANs (\cite{gans}) and VAEs (\cite{kingma2018variational}), they are trained using a very intuitive maximum likelihood loss function. Images and the latent vector, required to have a Gaussian distribution, correspond to flow models. Despite these intriguing characteristics, GANs and VAEs are utilized more frequently. This is due to the need for the Normalizing flow transformations to be invertible, significantly restricting the types of neural networks employed. For deployment in a real-world scenario, the invertible transformations must be efficiently calculable in the forward and sampling stages.

% Invertible convolutions have been essential for building expressive normalizing flow-based generative models since their introduction in Glow. Several attempts have been made to design invertible kk convolutions that are efficient in training and sampling passes. Though these attempts have improved the expressivity and sampling efficiency, they severely lag behind Glow, which uses only 1x1 convolutions regarding sampling time. Also, many approaches mask many parameters of the underlying convolution, resulting in lower expressivity on a fixed runtime budget. 


% A significant breakthrough came with Glow \cite{kingma2018glow} which used $1\times 1$ invertible convolutions to design normalizing flows. If it exists, the inverse function for a $1 \ 1\times 1$ convolution is also a $1\times 1$ convolution. Since computing $1 \times 1$ convolution has fast parallel algorithms for which running time does not depend on the spatial dimensions, they are also highly efficient in the forward pass (i.e., computing the latent vector from an image) as well as the sampling pass (i.e., computing the image from a sampled latent vector). Extending Glow to use invertible $k\times k$ convolutions promises to improve the expressivity further, allowing it to model more complex datasets. However, this is a challenging problem since the inverse function for a $k \times k$ convolution is generally given by a $n \times n$ matrix where $n = h \times w$ (i.e., a product of the spatial dimensions). Hence, while the forward pass can be fast, the trivial approach for the sampling pass will cost $O(n^2)$ operations per convolutional layer.

% There have been several attempts at designing invertible $k \times k$ convolutions that are efficient to compute in the forward and sampling passes. Glow model tries to create an invertible convolution but has the limitation of  $ 1\times 1$ and can not be generalized to $  n\times n$ invertible convolution. Emerging convolution \cite{hoogeboom2019emerging}, extended work of Glow proposed the chaining of autoregressive convolution and required two convolutions for the $n \times n$ convolution. \cite{hoogeboom2020convolution}  introduced a method for the invertible transformation by converting a linear transformation to an exponential transformation and then computing the Jacobian's determinant, but the sampling time is slow. CInC Flow \cite{nagar2021cinc} introduced a padded $3 \times 3$ convolution layer by giving it the necessary and sufficient conditions to make it invertible. We introduced a new flow step that uses the independence between the channels for the convolution matrix and does parallel computation to make sampling time faster.



% The idea of generative modeling stems from training a generative model whose sample comes from the same distribution as the training data distribution. Most of the generative models can be grouped as Generative adversarial networks (GANs) \cite{goodfellow2014generative}, Energy-based models (EBMs) \cite{zhang2022generative}, Variational autoencoders (VAEs) \cite{kingma2013auto, kingma2018variational}, Autoregressive models \cite{oord2016wavenet, nash2020polygen} and Flow-based models \cite{dinh2016density, hoogeboom2019emerging, kingma2018glow}. 
% An invertible neural network requires the inverse of the network with fast and efficient computation of the Jacobian determinant \cite{song2019mintnet}. Invertible neural networks can be used for generation and classification with more interpretability. \cite{kingma2018glow} proposed an invertible $1 \times 1$ convolution building on top of NICE \cite{dinh2014nice}  and RealNVP \cite{dinh2016density}, consisting of a series of flow steps combined in a multi-scale architecture. Each flow step consists of an actnorm followed by an invertible $1 \times 1$ convolution, followed by a coupling layer. Emerging Flows \cite{hoogeboom2019emerging} presented a method to generalize $1 \times 1$ convolution to invertible $ d \times d$ convolutions. Emerging flows chain two specific auto-regressive convolutions to form a single convolutional layer following the associativity of the convolution operation. Each of these auto-regressive convolutions is chosen such that the resulting convolution matrix $\mathbf{M}$ is triangular with inverse time of each of the convolutions is O$(H W k^2)$. \emph{MintNet} \cite{song2019mintnet} presented a method for designing invertible neural networks by combining building blocks with a set of composition rules. The inversion of the proposed blocks necessitates a sequence of dependent computations that increase the network's sampling time. \emph{SNF} \cite{keller2021self} proposed a method to reduce the computation complexity of the Jacobian determinant by replacing the gradient term with a learned approximate inverse for each layer. This method avoids the determinant of the Jacobian, makes it approximate, and requires an additional backward pass for inversion of the convolution. \emph{MaCow:} \cite{ma2019macow}. At the same time, many other papers make use of the invertibility of triangular matrices to reduce inversion time; MaCow outperforms all of them by performing the inverse in O$(H)$ or O$(W)$ by carefully masking $4$ kernels at the top, left, bottom, and right to achieve a full convolution. MaCow uses four autoregressive convolutions to make an effective standard convolution.\emph{Woodbury} \cite{lu2020woodbury} This paper employs the \emph{Woodbury transformation} for invertible convolution, which is a generalized permutation layer that models dimension dependencies along the channel and spatial axes using the channel and spatial transformation.


% \section{Generative modeling by estimating gradients of the data distribution}
% Introduce a new generative model in which samples are generated using Langevin dynamics and data distribution gradients computed by score matching. Because gradients can be ill-defined and complex to estimate when the data resides on low-dimensional manifolds, we perturb the data with various levels of Gaussian noise and estimate the corresponding scores, i.e., the vector fields of gradients of the perturbed data distribution for all noise levels. As the sampling process approaches the data manifold, we suggest an annealed Langevin dynamics with gradients corresponding to increasingly diminishing noise levels. Our system for flexible model designs does not need sampling during training or adversarial methods, and it provides a learning goal for principled model comparisons. On the CIFAR-10 dataset, our models create samples equivalent to GANs on the MNIST, CelebA, and CIFAR-10 datasets, achieving a new state-of-the-art inception score of 8.87. In addition, we demonstrate through picture inpainting studies that our models acquire useful representations \cite{song2019generative}.


% Quality assessment of agricultural produce is crucial in minimizing food stock wastage. However, this is done manually and requires expert supervision, especially in smaller seeds like corn. We propose a novel computer vision-based system for automating this process. We built a novel seed image acquisition setup, which captures both the top and bottom views. Dataset collection for this problem has data annotation costs/time and class imbalance challenges. We address these challenges by i.) using a Conditional Generative Adversarial Network (CGAN) to generate real-looking images for the classes with fewer images and ii.) Annotate a large dataset with minimal expert human intervention using a Batch Active Learning (BAL) based annotation tool. We benchmarked different image classification models on the dataset that we obtained. We can get an accuracy of up to 91.6\% % for testing seed samples' physical purity.



%%% Chapter-2


%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CInC Flow: Normalizing Flow Model with Invertible 3×3 CNN Layers
% \section{Introduction}
% Normalizing flows present a compelling alternative to GANs for generative modeling by enabling direct optimization of the dataset's maximum likelihood. Their architecture, based on invertible transformations, also facilitates the exact computation of a latent vector for any given image. However, the invertibility requirement restricts the use of standard, expressive neural network architectures like CNNs in normalizing flows. Previous efforts, such as emergent convolutions, addressed this by constructing invertible 3×3 CNN layers using pairs of masked CNN layers, which are computationally inefficient.

% In this work, we analyze and derive the necessary and sufficient conditions to achieve invertibility in padded 3×3 CNNs, enabling their use as expressive and efficient layers in normalizing flows. Our proposed conditions are straightforward and can be consistently maintained throughout the training process. Unlike emergent convolutions, which rely on two CNN layers for invertibility, our approach achieves this with only one CNN layer per invertible layer, significantly enhancing computational efficiency.

% We introduce a new coupling layer, Quad-coupling, which increases flexibility and expressiveness within normalizing flow architectures. Benchmark results demonstrate that our approach achieves comparable performance to emergent convolutions while improving model efficiency.

% The code for our method is available on GitHub\footnote{\label{footnote}\url{https://github.com/Naagar/Normalizing_Flow_3x3_inv}}.


% \subsection{Image Manipulation}
% Normalizing flows are invertible generative models. This invertibility property is advantageous for getting insight into the features learned by the model. We use this to modify images by acting on their latent representation. 

% To do this, we use a dataset containing images and their attributes (for instance, the Celeba dataset (\cite{celeba}), which includes images of faces as well as characteristics of these faces). Such a dataset can be modelled as two matrices: one $X\in\mathbb{R}^{N\times n}$ representing $N$ images of size $n$ and another $A\in\mathbb{R}^{N\times m}$ containing the $N$ corresponding annotations corresponding to $m$ attributes. After training a normalizing flow using only $X$, we can collect the output (although we could collect the activation of any given layer instead) as a matrix $Z\in\mathbb{R}^{N\times n}$. Then, after normalizing $A$ and $Z$, we can compute the covariance matrix between the attributes and the latent representation of our images $ C=A^TZ\in\mathbb {R}^{m\times n}$.

% Then to modify an image $x$ we compute it is latent representation $z$ and add $\alpha C_i$ where $C_i$ is the line in $C$ corresponding to the attribute we want to modify: $C_i\in\mathbb{R}^n$ is a vector indicating in which direction a latent representation should be modified to increase the attribute in the image space. Once this is done, we collect the model's output (although one could also collect the activations of any particular layer) for every input in our dataset. The attributes included in the dataset for every input make it possible to compute the covariance matrix of the output with respect to the attributes. 

% Each line of this matrix indicates which components should be increased or decreased to have the corresponding attribute in the input image. Conversely, each row indicates how each neuron will affect the characteristics of the image. Using this information, one can obtain the latent representation of an image, modify this representation to add or remove attributes, and then inverse the model to get the modified image.

% \begin{figure}[ht]
% 	\begin{center}
% 		\includegraphics[width=0.8\linewidth]{images/interp_grid.png}
% 	\end{center}
% 	\caption{We can see the result of the gradual interpolation of the more than two \emph{latent vector} \textbf{($z$)}. Ratio to which \emph{latent vector} \textbf{($z$)} is used to regenerate interpolated image is linear left to right.}
% 	\label{fig:interp_grid}
% \end{figure}
% \begin{align}
% z = \alpha_1 * z_1 + \alpha_2 * z_2 + \alpha_3 * z_3 + \alpha_3 * z_4
% \end{align}
% where $z_1$, $z_2$, $z_3$, $z_4$, are the \emph{latent vector} \textbf{($z$)} of corner images and $\alpha_1$, $\alpha_2$, $\alpha_3$, $\alpha_4$ $\in$ ($0$, $0.15$, $0.85$, $1$) are the fractions.   

% \begin{figure}[h]
% 	\begin{center}
% 			\includegraphics{images/pad.pdf}
% 	\end{center}
% 	\caption{The matrix corresponding to a convolution with a kernel of size three applied to an input of size $4\times4$ padded only on one side and with two channels.}
% 	\label{fig:pad_conv}
% \end{figure}
% \begin{figure}[h]
% 	\begin{center}
% 		\includegraphics{images/pad_trig.pdf}
% 	\end{center}
% 	\caption{The matrix corresponding to a convolution with a kernel of size three applied to an input of size $4\times4$ padded only on one side and with two channels. One of the weights of the kernel is masked. Note that the equivalent matrix M is \emph{triangular}.}
% 	\label{fig:triang_conv}
% \end{figure}

% \newpage
% \clearpage
% \begin{contributions} % will be removed in PDF for initial submission,
%                       % so you can already fill it to test with the
%                       % 'accepted' class option
%     Briefly list author contributions.
%     This is an excellent way of clarifying who did what and giving proper credit.

%     H.~Q.~Bovik conceived the idea and wrote the paper.
%     Coauthor One created the code.
%     Coauthor Two created the figures.
% \end{contributions}

% \begin{acknowledgements} % will be removed in PDF for initial submission,
%                          % so you can already fill it to test with the
%                          % 'accepted' class option
%     Briefly acknowledge people and organizations here.

%     \emph{All} acknowledgements go in this section.
% \end{acknowledgements}

% \bibliography{uai2021-template}

% \appendix
% % NOTE: necessary when ptmx or no mathfont class option is given
% \providecommand{\upGamma}{\Gamma}
% \providecommand{\uppi}{\pi}


% We also show that Theorem \ref{thm:inv-conv-1}  can be generalized to convolutions on arbitrary channels and window sizes. 
% They can be found in the supplementary material.

% \begin{theorem}[Characterization of Invertible Convolutions]
% $$M \text{ is invertible iff } \text{det}(K_{3,3}) \neq 0.$$
% \end{theorem}
% \begin{figure}[ht!] 
%     \centering
%     \includegraphics[width=0.95\linewidth]{images/kernal_matrix.png} 
%     \caption{Different types of padding: on the left the standard padding (the input is in green and the white part is added zeros) that give a matrix similar to Figure \ref{fig:m atrix}(a); on the right an alternative padding scheme that results in a block triangular matrix $M$ (see Figure \ref{fig: matrix}(b)).}
%     \label{fig:padding}
% \end{figure}
% \paragraph{Invertible Transformations:}
% Given an invertible function $f:X\to Y$, and a probability distribution $D$ on the input space $X$, the probability distribution of the random variable $f(X)$ (where $X$ is sampled from $D$) is given by:
% \[  p\left(f(x)\right)= p\left(x\right) \left|\frac{\partial f\left(x\right)}{\partial x^T}\right| ^{-1} \]
% where  $\left|\frac{\partial f\left(x\right)}{\partial x^T}\right|$ is the jacobian of f.
% Quad Coupling mechanism
%Experimental validation. Quality versus run-time concerning emergent.

% Clearly, there are intermediate choices: one can split the input into K
% parts and transform the k-th part element-wise as a function of parts 1 to k-1, with K = 2
% corresponding to a coupling layer and K = D to a fully autoregressive flow. Using masking,
% inverting the transformation will be O(K) times more expensive than evaluating it, hence
% K could be chosen based on the computational requirements of the task.

% Coupling transforms solve two critical problems for normalizing flows: they have a tractable
% Jacobian determinant, and they can be inverted exactly in a single pass.



%% Chapter-3


% \section{Intro}
% \section{Results}
%%%%%%%%%%%%%%%%%% TRASH      TRASH TRASH
%%%%%%%%%%%%                 TRASH 
% \begin{figure}
%     \centering
%     \includegraphics[width=0.99\textwidth]{}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=0.99\textwidth]{Images/Fig-Chap3/FInCFlow_model.pdf}
%     \caption{Overview of our proposed FInC Flow model \cite{nagar2023fincflow}.}
%     \label{fig:fincflow}
% \end{figure}

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.99\textwidth]{Images/Fig-Chap3/celeba_reconstruct.pdf}
%     \caption{Reconstructed sample images after the model was trained on the CelebA dataset.}
%     \label{fig:celeba_reconstruct}
% \end{figure}

% In each iteration of the algorithm \ref{alg:inv_algo}, we can compute the inverse for every element on the diagonal of the image. Since there are $H + W - 1$ secondary diagonals in a matrix and there are at maximum $k^2$ entries in a row, the time complexity will be

% \begin{equation}
% \underbrace{(1 + 1  + \cdots+1)}_{H + W - 1 \text{ times}} k^2 = (H + W-1) k^2
% \end{equation}


% The $(i, j)^{th}$ pixel value of the output $Y$ can be calculated as 
% $$
% y_{i, j} = (\textbf{M}_{iW+j, :})^T \cdot x
% $$ 
% which means $y_{i,j}$ is the dot product of $\textbf{M}_{iW+j, :}$ i.e., the corresponding row of matrix $\textbf{M}$ and the vectorized input $x$.
% Because $\textbf{M}$ is lower triangular, $y_{i,j}$ depends only on the values of $x_{\le i, \le j}$ where $x_{\le i, \le j}$ are the pixels that are on the top and left side of the pixel $(i, j)$ including $(i, j)$.
% Because all the diagonal values are $w_{k, k}$, we have, 
% \begin{align*}
% y_{i, j} &= w_{k, k} x_{i, j} + f(x_{<i, <j})\\
% x_{i, j} &= \frac{y_{i, j} - g(x_{<i, <j})}{w_{k, k}}
% \end{align*}
% where $(<i, <j)$ are the pixels which are strictly top and left side of $(i, j)$, Following the masking pattern of CInC Flow, we have $w_{k, k} = 1$ and $f$ is a linear function which is given by weighted sum of the given pixels weighed by the filter values. So,
% \begin{equation}
% \label{eq:inv_convolution}
% x_{i, j} = y_{i, j} - \sum_{p=0}^{k} \sum_{q=0}^{k} x_{i-p, j-q} K_{p, q}  
% \end{equation}
% where  $p = q \neq 0$. 
% We extend Equation \ref{eq:inv_convolution} for multiple channels and present it in Line 8 of Algorithm \ref{alg:inv_algo}. 

% $$
% \underbrace{(1 + 1  + \cdots+1)}_{H + W - 1 \text{ times}} k^2 = (H + W-1) k^2
% $$

% We use the $3 \times 3$ Invertible Convolutional Block introduced in CInC Flow \citep{nagar2021cinc}. We refer to this block as "Padded Conv. Block". 
% \paragraph{Algorithm:}\label{sec:algorithm}
% % going back from latent space to data space, the inversion of the FInC Flow unit uses the independence of the channels contributing to the convolution matrix, see Figure \ref{fig:conv_parallel}a. The inverse of the convolution is implemented as represented in the Algorithm 
% Our Fast Parallel Inversion Algorithm to inverse a \emph{TL} padded input is given in Algorithm \ref{alg:inv_algo}. 


% \begin{equation} \label{eq:convolution_matrix}
%     \mathbf{y} = \mathbf{M} \mathbf{x}
% \end{equation}
%define matrix of the convolutions, its dimensions


% \begin{equation} \label{eq:conv_inverse}
%     \mathbf{x} = \mathbf{M}^{-1} \mathbf{y}
% \end{equation}
% \begin{equation}

% \begin{split}

% \end{split}
% \end{equation}

% \begin{equation}

% \begin{split}
% x_{i, j+1} &= y_{i, j+1} - f(x_{<i, <j+1}) \\
% &=y_{i, j+1} - \beta x_{i, j} - f_2(x_{<i, <j})
% \end{split}
% \end{equation}




% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=0.99\linewidth]{fig/conv_matrix_explain.pdf}
%     \caption{Visualization of the convolution for the padded input ($4 \times 4 \times 2$) and masked filter ($2 \times 2 \times 2 \times 2$), and the size of the output is the same as the input.}
%     \label{fig:conv_matrix_explain}
% \end{figure}

% \begin{figure*}[!ht]
%     \centering
%     % \vspace{-2em}
%     \includegraphics[width=0.99\linewidth]{fig/conv_matrix.pdf}
%     % \vspace{-01em}

%     \caption{(a) Convolution matrix  ($M$): obtained after convolution of a $4 \times 4 \times 2$ image with a $2 \times 2 \times 2$ masked filter. (b) Convolution Matrix $M$ obtained for a $4 \times 4 \times 2$ image with a $2 \times 2 \times 2 \times 2$ filter. (c)Parallel Computation in a $6 \times 6$ Image. Pixels with the same color have their inverses calculated in parallel.}
%     \label{fig:conv_matrix}
%     % \vspace{-01em}
% \end{figure*}

% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=0.99\linewidth]{AISTATS2023PaperPack/fig/celeba_generated.pdf}
%     % \vspace{-0.4em}
%     \caption{Generated image samples after training FInC Flow for  $200$ epochs on CelebA64 dataset.}
%     % \vspace{-01em}
%     \label{fig:celeba64_generated}
% \end{figure}

% CinCFlow, MaCow Woodbury, Flow++, Glow, Emerging, 
% In Figure \ref{fig:mnist}, we present the effectiveness of the  FInC Flow model in the reconstruction (sampling) of the images and compare with SNF \citep{keller2021self} reconstructed samples. First, we feed the input image to the forward flow and learn the features ($z$). To reconstruct the images from the latent vector ($z$), give the $z$ as input to the inverse flow and calculate the reconstruction difference (see Figure \ref{fig:mnist}ii). To show the interpretability of our Flow model, we used the CelebA dataset \citep{liu2015faceattributes} consists of images with faces and attributes corresponding to these faces. Figure \ref{fig:cifar10_reconstruct}a presents the reconstructed face images for the CelebA dataset after training our model for $200$ epochs, and for CIFAR10 see Figure \ref{fig:cifar10_reconstruct}b.

% \begin{figure*}[!h]
%     \centering
%     \includegraphics[width=0.99\linewidth]{fig/reconstruct_snf_and_our.pdf}
%     \vspace{-1em}
%     \caption{The visualization of the image reconstruction difference for the  (a) SNF \citep{keller2021self} and (b) FInC Flow (our). Going forward, and learning the features ($z$). Next, from the learned features ($z$), the images are generated using the latent vector and going back from the latent space to the data space. (i) original image from dataset, (ii) reconstruction difference, (iii) reconstructed image samples.}
%     \label{fig:mnist}
% \end{figure*}




% \begin{figure} 
%     \centering
%     \subfloat[\label{2a}]{%
%       \includegraphics[width=0.333\linewidth]{mnist_original_samples.pdf}}
%     \hfill
%     \subfloat[\label{2b}]{%
%         \includegraphics[width=0.333\linewidth]{mnist_reconstruction_difference.pdf}}
%     \hfill
%     \subfloat[\label{2c}]{%
%         \includegraphics[width=0.333\linewidth]{mnist_reconstructed_samples.pdf}}
%   \caption{The visualization of the image reconstruction difference: going forward and learning the features ($z$). Next, from the learned features ($z$), the images are generated using the latent vector and going back from the latent space to the data space. (a) original image from the dataset, (b) reconstruction difference, (c) generated images.}
%   \label{fig:mnist} 
% \end{figure}



% \vspace{10em}



% \begin{figure}
%     \centering
%     \includegraphics[width=0.99\textwidth]{}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=0.99\textwidth]{Images/Fig-Chap3/FInCFlow_model.pdf}
%     \caption{Overview of our proposed FInC Flow model \cite{nagar2023fincflow}.}
%     \label{fig:fincflow}
% \end{figure}

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.99\textwidth]{Images/Fig-Chap3/celeba_reconstruct.pdf}
%     \caption{Reconstructed sample images after the model was trained on the CelebA dataset.}
%     \label{fig:celeba_reconstruct}
% \end{figure}

% \begin{equation*}
%     \begin{bmatrix}
%     w_{22} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\
%     w_{21} & w_{22} & 0 & 0 & 0 & 0 & 0 & 0 & 0\\
%     0 & w_{21} & w_{22} & 0 & 0 & 0 & 0 & 0 & 0 \\
%     w_{12} & 0 & 0 & w_{22} & 0 & 0 & 0 & 0 & 0 \\
%     w_{11} & w_{12} & 0 & w_{21} & w_{22} & 0 & 0 & 0 & 0 \\
%     0 & w_{11} & w_{12} & 0 & w_{21} & w_{22} & 0 & 0 & 0 \\
%     0 & 0 & 0 & w_{12} & 0 & 0 & w_{22} & 0 & 0  \\
%     0 & 0 & 0 & w_{11} & w_{12} & 0 & w_{21} & w_{22} & 0\\
%     0 & 0 & 0 & 0 & w_{11} & w_{12} & 0 & w_{21} & w_{22} \\
%     \end{bmatrix} 
%     \times
%     \begin{bmatrix}
%     x_{11} \\
%     x_{12} \\
%     x_{12} \\
%     x_{21} \\
%     x_{22}  \\
%     x_{23} \\
%     x_{31} \\ 
%     x_{32} \\ 
%     x_{33}\\
%     \end{bmatrix}

% \end{equation*}

% \begin{NiceTabular}{ccc}[hvlines]
% \CodeBefore
% \cellcolor{red!10}{1-1}
% \cellcolor{green!10}{1-2,2-1}
% \cellcolor{yellow!10}{1-3,2-2,3-1}
% \cellcolor{blue!10}{2-3,3-2}
% \cellcolor{cyan!10}{3-3}
% \Body
% $x_{11}$ & $x_{12}$ & $x_{13}$ \\
% $x_{21}$ & $x_{22}$ & $x_{23}$ \\
% $x_{31}$ & $x_{32}$ & $x_{33}$ \\
% \end{NiceTabular}
% $\ast$
% \begin{NiceTabular}{cc}[hvlines]
% $w_{11}$ & $w_{12}$\\
% $w_{21}$ & $w_{22} $
% \end{NiceTabular}
% $=$

% $\begin{bNiceArray}{ccccccccc}
% \CodeBefore
% \rowcolor{red!10}{1}
% \rowcolor{green!10}{2,4}
% % \rowcolor[HTML]{03FCF0}{3,5,7}
% \rowcolor{yellow!10}{3,5,7}
% \rowcolor{blue!10}{6,8}
% \rowcolor{cyan!10}{9}
% % \resizebox{\textwidth}{!}{
% \Body

% w_{22} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\
% w_{21} & w_{22} & 0 & 0 & 0 & 0 & 0 & 0 & 0\\
% 0 & w_{21} & w_{22} & 0 & 0 & 0 & 0 & 0 & 0 \\
% w_{12} & 0 & 0 & w_{22} & 0 & 0 & 0 & 0 & 0 \\
% w_{11} & w_{12} & 0 & w_{21} & w_{22} & 0 & 0 & 0 & 0 \\
% 0 & w_{11} & w_{12} & 0 & w_{21} & w_{22} & 0 & 0 & 0 \\
% 0 & 0 & 0 & w_{12} & 0 & 0 & w_{22} & 0 & 0  \\
% 0 & 0 & 0 & w_{11} & w_{12} & 0 & w_{21} & w_{22} & 0\\
% 0 & 0 & 0 & 0 & w_{11} & w_{12} & 0 & w_{21} & w_{22} \\
% % }
% \end{bNiceArray}$

% $\begin{bNiceArray}{c}
% % \CodeBefore
% % \rowcolor{red!10}{1}
% % \rowcolor{green!10}{2,4}
% % % \rowcolor[HTML]{03FCF0}{3,5,7}
% % \rowcolor{yellow!10}{3,5,7}
% % \rowcolor{blue!10}{6,8}
% % \rowcolor{cyan!10}{9}
% % \Body
% x_{11} \\
% x_{12} \\
% x_{12} \\
% x_{21} \\
% x_{22}  \\
% x_{23} \\
% x_{31} \\ 
% x_{32} \\ 
% x_{33}\\
% \end{bNiceArray}$


% \subsection{Efficient and Fast Inversion:  comparison to other approaches}

% 

% \begin{algorithm}
% \caption{Fast Parallel Inversion Algorithm}
% \KwIn{$K$ - Convolution Kernel, $X$ -  Output of the Convolution}
% \KwResult{$Y$ -  Input to the Convolution / Inverse of the Convolution}
% \textbf{Initialization:} $Y \gets X$ \;
% %%$d \gets $ H + W - 1\;
% \For{$d \gets 1, H + W - 1$}{
% %   instructions\;
% %   \eIf{condition}{
% %   instructions1\;
% %   instructions2\;
% %   }{
% %   instructions3\;
% %   }
%     \For {$c \gets 0, C - 1$}{
%         \Comment{The below lines of code execute in parallel on different threads on the GPU for every pixel (c, h, w) on the diagonal index $d$}
        
%         \For{$k_h \gets 0, k_H - 1$}{
%           \For{$k_w \gets 0, k_W - 1$}{
%           \For{$k_c \gets 0, C - 1$}{
%           \If{pixel $(k_c, h - k_h, w - k_w)$ not out of bounds}{
%              $Y[c, h, w]$ \gets
%          $Y[c, h, w] -$ \\
%          $Y[k_c,h - k_h, w - k_w] * K[c, k_c, k_H - k_h - 1, k_W - k_w - 1]; $
%           }
%           }
%           }
%         } 
%     }
%     \Comment{synchronize all threads}
%  }
%  \label{alg:inv_algo}
% \end{algorithm}

% $M$ is \emph{lower triangular} and can be inverted as presented in CInC Flow. The blank(white) entries represent zero, and the colored entries are non-zero (making sure all the diagonal values, colored as black, are also non-zero). Observing the fact that every $8 \times 8$ blocks get repeated diagonally, we use this fact to compute the inverse of this convolution matrix and parallelize it for each color.


% \begin{figure}
%     \centering
%     % \subfloat[\label{64x4x2_toeplitz_matrix} Matrix $M$]{%
%     %     \includegraphics[width=0.316\linewidth]{toeplitz_matrix.pdf}}
%     % \subfloat[\label{Toeplitz}]{%
%     %   \includegraphics[width=0.35\linewidth]{fig/3x3tl.png}}
%     % \subfloat[\label{6x6_Parallel}]{%
%     \includegraphics[width=0.99\linewidth]{fig/parallel_conv.pdf}
%         % }
%     \vspace{-0.4em}
%     \caption{(a) Convolution Matrix $\mathbf{M}$ obtained for a $4 \times 4 \times 2$ image with a $2 \times 2 \times 2 \times 2$ filter. White spaces in the matrix represent $0$, and the colored values represent non-zero values.  $\mathbf{M}$ is a lower triangular matrix. Visualization of parallel computation. (b) Convolution matrix  ($M$): obtained after convolution of a $4 \times 4 \times 2$ image with a $2 \times 2 \times 2$ masked filter. $M$ is \emph{lower triangular} and can be inverted as presented in CInC Flow \citep{nagar2021cinc}. The blank(white) entries represent zero, and the colored entries are non-zero (making sure all the diagonal values, colored as black, are also non-zero). Observing the fact that every $8 \times 8$ blocks get repeated diagonally, we use this fact to compute the inverse of this convolution matrix and parallelize it for each color. (c) Diagonal Matrix ($D$): represents the parallel computation of the matrix $M$ for an input $6 \times 6$; the inverse of pixels with the same color are computed in parallel.}
%   \label{fig:parallel_conv} 
% \end{figure}

% \begin{figure}[!h]
%     \centering
% %   \subfloat[FInC Flow Step\label{3a}]{%
% %   \vspace{4em}
%     %   \includegraphics[width=0.30\linewidth]{fastflow_oneStep.pdf}}
% %   \hfill
% %   \subfloat[Multi-scale architecture\label{3b}]{%
%     \includegraphics[width=0.88\linewidth]{fig/architecture_FFStep_arch.pdf}
%     % }
%     \vspace{-0.4em}
%     \caption{We propose a FInC Flow architecture  \ref{section:fastflowunit} where each FInC Flow step (left) consists of an actnorm step, followed by an invertible 1 × 1 convolution, followed by a coupling layer. This flow is combined with a multi-scale architecture \ref{subsec:arch} (right).}
%     \label{fig:fastflow2}
% \end{figure}

% \section{Parallel Inversion Algorithm}


% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=0.45\linewidth]{fig/toeplitz_matrix.pdf}
%     \caption{Convolution Matrix $\mathbf{M}$ obtained for a $4 \times 4 \times 2$ image with a $2 \times 2 \times 2 \times 2$ filter. White spaces in the matrix represent $0$, and the colored values represent non-zero values.  $\mathbf{M}$ is a lower triangular matrix}
%     \label{fig:4x4x2_toeplitz_matrix}
% \end{figure}
% Woodbery Tranforms, MaCow,


% Normalizing flows have also been used for density estimation, variational inference, and generative modeling. Previous work on Normalizing flow, Non-linear Independent Component Estimation (NICE) \citep{dinh2014nice}, applies flow-based models for modeling complex high-dimensional densities. RealNVP \citep{dinh2016density} extended NICE with a more flexible invertible transformation to experiment with images. Glow \citep{kingma2018glow} as a generative flow with invertible $ 1 \times 1$ $ convolutions significantly improved the density estimation performance. The extension of Glow, Emerging \citep{hoogeboom2019emerging} generalize  $ 1 \times 1 $ to  $ d \times d $ by padding the input and masking the kernel, but for one standard convolution, Emerging need two convolutions. 


% Let $ f: \mathbb{R} ^{d} \rightarrow \mathbb{R} ^{d} $ with inverse $ f^{-1} = g $, i.e. the composition $g \cdot f(z)$, where $z$ is the latent vector (a random variable) with distribution $q(z)$, resulting random variables $z^{'} = f(z) $ has a distribution: 
% \begin{equation}
%     q (z^{'}) = q(z) \left| \det \frac{\delta f^{-1}}{\delta z^{'}}\right| = q(z) \left| \det \frac{\delta f}{ \delta z}\right|^{-1}
% \end{equation}

% where right equality can be seen by applying the chain rule and its property of \emph{Jacobian} of an invertible function. 


%%%% Chapter-4

%%%%%%%%%%%%%%%%%%%%%%%%

% Trash 
% 

% Sampling with Emerging convolutions is slow because of its autoregressive nature. Both SNF and Inverse-Flow are efficient in training and sampling. We observe that Inverse-Flow performs significantly better in terms of sampling time as well as training time. Our scores are worse than those reported by \citep{keller2021self} because we use smaller models and train each model on a single GPU. Furthermore, for smaller models ($L = 2$, $K = 4$), the contribution of inv-conv becomes more important, as evidenced by improved performance (see Table-\ref{tab:if_M_st_2_4}, \ref{tab:M_st_2_4}).


% \paragraph{Complexity Analysis:} 

% \begin{algorithm}[!t] 
%     \caption{ Algorithm of Inv-Conv }
%     \label{alg:inv_algo}
%     \KwIn{$K$: Kernel of shape $(C, C, k_H, k_W)$\\
%     $Y$: output of the conv of shape $(C, H, W)$}
%     \KwResult{$X$: inverse of the conv. with shape $(C, H, W)$.}
%     \textbf{Initialization:} $X \gets Y$ \;
%     \For{$d \gets 0, H + W - 1$}{
%         \For {$ c \gets 0, C - 1 $}{
%             \Comment{The below lines of code execute in parallel on different threads on the GPU for every index $(c, h, w)$ of $X$  on the $d$th diagonal.} 
            
%                 \For{$ k_h \gets 0, k_H - 1 $}{
%                 \For{$ k_w \gets 0, k_W - 1 $}{
%                 \For{$ k_c \gets 0, C - 1 $}{
%                     \If{pixel $ (k_c, h - k_h, w - k_w) $ not out of bounds}{
%                          $ X[c, h, w]  \gets X[c, h, w] - X[k_c,h - k_h, w - k_w] * K[c, k_c, k_H - k_h - 1, k_W - k_w - 1]; $
%                       }
%                 }
%                 }
%                 } \Comment{synchronize all threads}
%         } 
%      }
% \end{algorithm}


% In this paper, we give a fast and efficient backpropagation algorithm for the inverse of convolution. We proposed a flow-based model, Inverse-Flow, that leverages the convolutions for efficient sampling and the inverse of the convolution for learning. Our work makes several key contributions to the field of generative modeling:

% \begin{enumerate}
%     \item We proposed a fast backpropagation algorithm for the inverse of convolution, leveraging the independence and parallelization operations to improve fast training with faster sampling.
%     \item We developed a multi-scale Inverse-Flow architecture that significantly accelerates the sampling process in flow models. 
%     \item We provided a GPU (CUDA) implementation of Inverse-Flow and its corresponding backpropagation algorithm, enabling high-performance computation on modern hardware.
%     \item We conducted extensive experiments to demonstrate the training capabilities of Inverse-Flow and its substantial improvements in sampling time compared to traditional flow models.
% \end{enumerate}

% Our results demonstrate that the inverse of convolution can be effectively trained and utilized for both sampling and training. The GPU implementation of the backpropagation for the inverse of convolution facilitates rapid training and significantly faster sampling within the flow-based model architecture. Notably, we achieved substantial improvements in sampling time for normalizing flow models and positioning flow-based approaches as competitive alternatives to other generative models such as diffusion models, GANs, and vision transformers. Furthermore, our efficient backpropagation algorithm for inverse convolution opens new possibilities for training more expressive and faster-flow models. This advancement has the potential to broaden the applicability of flow-based models across various domains in computer vision and beyond.

% We have made our implementation of Inverse-Flow, along with baselines and experimental code, a publicly available repository. The GPU implementation is optimized for performance through parallelization via the PyTorch Ninja frameworks. In conclusion, Inverse-Flow represents a significant step forward in the development of efficient and expressive generative models. By addressing key computational challenges in flow-based models, our work contributes to the ongoing advancement of generative models and their practical applications in real-world scenarios.

%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%
% \section{Conclusion}

% Inverse-Flow implementation shows proof that the inverse of a convolution can be trained and used for sampling and inference. The GPU implementation of the backpropagation for inverse convolution fast training and faster sampling using the flow-based model architecture. We show a big improvement in the sampling time for the Normalizing flow models and put the flow model in competition with other generative models such as Diffusion, GANs, and Vision transformers. The backpropagation algorithm algorithm for the inverse convolution a new set of possibilities for training fast and more expressive Flow models. 


%%% Chapter-5

%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%

% \paragraph{Batch Active Learning (BAL) for Fast Annotation:} \label{sec:active-learning} Data efficiency is a crucial problem in Deep Learning. Active learning, a subfield in Machine learning, is centered around attaining data efficiency. To avoid the tedious data labeling of a large dataset, we iteratively query the most informative points from a set of unlabeled points in Active Learning. However, in practical Active learning, we query a batch of points from an unlabeled set of the most informative and diverse points rather than acquiring single points. The question is which subset of points of the unlabeled set should be added to the training set so that the model would learn the fastest when trained on this updated training set than picking any other subset of the unlabeled points. 

% Moreover, since we can label multiple images in a single screen shown as a grid to the annotator (see Fig \ref{fig:anno_ui}), sampling points belonging to the same class of the underlying distribution are possible. In such a scenario, we will have an accurate model in one class but not in all other classes. We query the least confidence to avoid this situation, and the queried set should be diverse. Batch Active Learning (BAL) was proposed to solve such problems, which we use to build an annotation tool.
% \paragraph{Batch Active Learning (BAL):}\label{subsec:batch} We start with the corn seed \emph{primary} dataset with 17,802 images and do a 90\%-10\% train-validation split to train the BAL model. We also have an unlabeled dataset of corn seeds, 26,777, to label using BAL. Specifically, we use the BatchBALD \cite{BatchBALD} method.  An active learning cycle involves retraining a model on the data annotated so far. During training, we use early stopping to avoid over-fitting. The used acquisition function is based on model uncertainty and ensures that the queried images are diverse in the predicted distribution model's uncertainty entropy. Next, pick  5000 images that have the highest entropy (most informative points). To ensure diversity, perform k-means clustering on these 5000 images until stabilization to find the 1000 cluster centers. After that, find the points closest to each of these 1000 centers in the dataset. This spits out 1000 images queried by the above acquisition function, along with their predicted labels. We then render these images and their predicted labels via an annotation tool that we have built for human annotation (see Figure \ref{fig:anno_ui}). Next step, the training set is updated by accumulating these images and the labels that the annotator makes. A reinitialized model is then trained on the updated training set, and the cycle continues.
% \vspace*{-\baselineskip}
% \begin{figure}[ht!]
%     \centering
%     % \vspace{-1em}
%     \includegraphics[width=0.99\linewidth]{Images/Fig-Chap5/ui_high_res_cropped.png}
%         % \vspace{-1.5em}
%     \caption{The user interface of the annotation tool. A single screen shows a batch of images.  If the suggestion is wrong, the user can relabel it. After a few active learning cycles, the model suggestions become more accurate, resulting in less effort from the annotator. Purple box: label suggested by the model.}
%     \label{fig:anno_ui}
%     % \vspace{-1em}
% \end{figure}

% \begin{figure}[ht!]
%   \centering
%   \includegraphics[width=0.99\linewidth]{Images/Fig-Chap5/batch_learning_cropped.png}
%   % \vspace{-1.5em}
%   \caption{(Left) Over 8 AL cycles shows an increase from 46.83 to 73.97\% % accuracy. (Right) Time taken to annotate shows a drastic decrease in annotation time over 8 AL cycles.}
%   \label{fig:batch_learning}
%   % \vspace{-2em}
% \end{figure}
% We record the validation accuracy for every cycle and find that with labeling only 9000 images of the 26,777 original unlabeled set, there is a significant increase in the validation accuracy from 46.83\% to 73.97\%, which is shown in Figure \ref{fig:batch_learning}.
% Moreover, the annotation time taken to annotate the first queried batch of 1000 images fell drastically from 1266.42 seconds to 682.02 seconds (which is the time taken to annotate the $8$th queried batch) as reflected in Figure \ref{fig:batch_learning}, thereby decreasing the annotation cost and efficiency significantly. After the $9$th cycle, the total labeled instances in the dataset are 26802 after adding new labeled images. 
% \vspace*{-\baselineskip}

%%% Chapter-6



%%%%%%%%%%%%%%% TRASH %%%%%%%%%%%%%%%%%%%

% For face anonymization, we employed the Inpaint-Anything model, a robust generative inpainting framework designed to fill masked regions with contextually appropriate content. Our approach first detected faces in each image using the RetinaFace \cite{deng2019retinaface} detection model, which provided precise bounding boxes around facial regions. We then applied inpainting exclusively within these bounding boxes, effectively removing identifiable facial features while preserving the surrounding visual context. This targeted anonymization strategy ensures that the core scene content remains unaltered, making it particularly suitable for privacy-preserving datasets in tasks like face detection or person re-identification without significantly compromising dataset utility.

% We used the IDD dataset and applied face detection to filter images without faces. After filtering, the training set has 608 images, and the validation set has 153 face images. Our train dataset contains 608 images with 3100 faces replaced with the Inpaint-Anything model \cite{yu2023inpaint}. The test dataset contains 153 images with 889 real faces for validation.

% Similarly, for the ECP dataset, we get 7712 images in the train set and 1533 in the test set. Test set images have a total of 3509 real faces. 

% \section{Results}

% Privacy preservation in autonomous driving data is rapidly becoming a critical challenge. As machine learning plays an increasing role in autonomous vehicle technology, companies and research groups have begun collecting vast data for development and validation. For instance, Waymo has accumulated over 5 million miles of driving data since 2018, and Cruise logged more than 770,000 miles in 2020 alone. This surge in data collection heightens the responsibility to ensure data privacy, especially for data gathered on public roads, which must adhere to privacy regulations such as the European GDPR, California CCPA, China’s CSL, and Japan’s APPI. These regulations mandate the protection of personal identifiable information (PII) within the data, including the right to request the removal of such information.

% In response, several commercial products now offer data de-identification solutions, typically through techniques like blurring. Examples include Brighter AI, Facebook Mapillary, and UAI Anonymizer, which anonymize faces and license plates, and Celantur, which extends this to entire human bodies and vehicles. Despite these advancements, the lack of accessible labeled datasets and baseline models remains a bottleneck for innovation in anonymization for autonomous driving. While commercial systems rely on private datasets for training and evaluation, the academic community has yet to address the need for open-source resources fully. To our knowledge, no public dataset currently exists that provides annotations for face and license plate detection specifically tailored to autonomous driving scenarios, leaving a significant gap in support for privacy-preserving research in this field.

% \begin{figure}[!ht]
%      \centering
%      % \begin{subfigure}[b]{0.3\textwidth}
%      %     \centering
%      %     \includegraphics[width=\textwidth]{figures/inpaint_sample_1.png}
%      %     % \caption{$y=x$}
%      %     \label{fig:y equals x}
%      % \end{subfigure}
%      % \hfill
%      \begin{subfigure}[b]{0.49\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Images/Fig-Chap6/inpainting_sample_04.png}
%          % \caption{$y=3\sin x$}
%          \label{fig:sample_03}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.49\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Images/Fig-Chap6/inpainting_sample_05.png}
%          % \caption{$y=5/x$}
%          \label{fig:sample_04}
%      \end{subfigure}
%         \caption{Image inpainting samples for the ECP dataset \cite{braun2018eurocity} images.}
%         \label{fig:samples2}
% \end{figure}
% \begin{figure}[!ht]
%     \centering
    
%     \includegraphics[width=\textwidth]{Images/Fig-Chap6/inpainting_sample_04.png}
    
%     \caption{Image inpainting samples for the ECP dataset \cite{braun2018eurocity}  images.}
%     \label{fig:samples2}
% \end{figure}

% \begin{figure}[!ht]
%     \includegraphics[width=\textwidth]{Images/Fig-Chap6/inpainting_sample_05.png}
%     \caption{Image inpainting samples for the ECP dataset \cite{braun2018eurocity}  images.}
%     \label{fig:samples3}
% \end{figure}





% A naive approach towards privacy preserving is via obfuscation, such as face blurring \cite{ilia2015face} while uploading to the cloud database. Rajput et al. \cite{rajput2020privacy} added Gaussian noise into the underlying image before applying down-sampling for obfuscation.

% \begin{figure*}[!ht]
%      \centering
%     \includegraphics[width=0.99\linewidth]{Images/Fig-Chap6/fF_val_batch1_pred.jpg}
%     \caption{Predicted bbox for faces with confidence and class using RetinaFace \cite{deng2019retinaface} for Pvt-IDD dataset.}
%     \label{fig:pred_labels2}
% \end{figure*}

% On the other hand, the scarcity of labeled datasets and baseline models, or the lack thereof, is impeding innovation and progress in solving the anonymization problem in autonomous driving. The commercial systems mentioned above generally do not have publicly accessible training and evaluation datasets. Meanwhile, the academic research community has paid less attention to this problem. To our knowledge, no public dataset for face detection for autonomous driving use cases is anonymized. For example, there are many public face detection datasets, such as PASCAL FACE, FDDB, UFDD, MALF, and WIDER FACE \cite{everingham2015pascal}, \cite{jain2010fddb}, \cite{nada2018pushing}, \cite{yang2015fine}, \cite{yang2016wider}.



%%% Chpater-7

% \section*{Code and Data Availability}
% The Python code and datasets used to implement the framework are available at \url{https://github.com/sydney-machine-learning/autoencoders_remotesensing}.


%% Chpater-8

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% -------------------------------------------------------------
% \paragraph{Change of Variables:} Let x and z be random variables which are related by a mapping 
% $ f: \mathbb{R}^n \rightarrow \mathbb{R}^n$ such that $ X = f(Z)$ and $ Z = {f}^{-1}(X)$. 
% Then 
% \begin{equation}
% p_x(x) = p_z({f}^{-1} | det(\frac{ \partial {{f}^{-1}(x)}}{\partial {x}}) |
% \end{equation} 

% where $x$ and $x$ have same dimension. $p_x$ is data distribution and $p_z$ is target distribution.

% \begin{algorithm}
% 	\caption{Affine-net}
% 	\label{alg:cap}

% 	\begin{algorithmic}
% 		%\KwInput x[B, C, h, w] 
% 		\Require input = x[c, h, w] %$n \geq 0$
% 		\Ensure $y = x^n$
% 		\State $y \gets 1$
% 		\State $X \gets x$
% 		\State $N \gets n$
% 		\While {$N \neq 0$}
% 		% \If{$N$ is even}
% 		% 	\State $X \gets X \times X$
% 		% 	\State $N \gets \frac{N}{2}$  \Comment{This is a comment}
% 		% \ElsIf{$N$ is odd}
% 		% 	\State $y \gets y \times X$
% 		% 	\State $N \gets N - 1$
% 		% \EndIf
% 		\EndWhile
% 	\end{algorithmic}

% \end{algorithm}

%\begin{algorithm}
%\STATE x_1, x_2 = split(x)

%\IF permute
%\ELSE 

%\end{algorithm}


% \emph{permute = True} (Eq-\ref{eqn_0}) when 
% \begin{equation} \label{eqn_0}
% 	i\_block \% 2 = 0
% \end{equation}
% %\algorithm
% \emph{permute = False}  (Eq-\ref{eqn_1}) when
% \begin{equation} \label{eqn_1}
% 	i\_block \% 2 = 1
% \end{equation}
% and 

% \begin{equation}
% 	z = concat(z_1, z_2)
% \end{equation}


% \begin{figure}[!pht]
% 	\centering
	
% 	\includegraphics[width=1\linewidth ]{figures/affine_sr_coupling_layer.pdf}
% 	\label{coup_graph}
% 	\caption{Computational graph of a Affine Coupling layer, where $s$ and $t$ are the convolution outputs \ref{eqn_1}.}
 
% \end{figure}

% \begin{figure}[!pht]
% 	% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
% 	% \includegraphics[scale=0.9\linewidth ]{test.pdf}
% 	\includegraphics[width=1\linewidth ]{figures/val_loss_affineVQ_vs_VQGAN.png}
% 	\caption{Val total loss (rec-loss, nll-loss, and ae-loss) plot affine-VQGAN vs VQGAN (taming transformers, AE used in ResShift) for training 50 epochs.}
% 	\label{fig:val_loss_affineVQ_vs_VQGAN}
% \end{figure}


% \begin{table*}[ht]
% 	\centering 
% 	\caption{ sample table, dummy values.}
% 	\begin{tabular}{c|c|ccccc|c} \toprule
% 		Dataset & Metrics & RealSR & BSRGAN & SwineIR-GAN & LDM & StableSR & Affine-StableSR \\ \midrule
% 		1  & 16.128 & 8.872 & 16.128 & 1.402 & 1.373 & 146.6 & 137.6 \\
% 		2  & 3.442  & 2.509 & 3.442  & 0.299 & 0.343 & 133.2  & 152.4  \\
% 		3  & 1.826  & 0.363 & 1.826  & 0.159 & 0.119 & 168.5  & 161.1 \\
% 		4  & 0.993  & 0.429 & 0.993  & 0.086 & 0.08  & 25.6   & 90     \\ \midrule
% 		5  & 1.29   & 0.099 & 1.29   & 0.112 & 0.097 & 175.6 & 114.7 \\
% 		6  & 0.483  & 0.183 & 0.483  & 0.042 & 0.063 & 22.3   & 122.5  \\
% 		7  & 0.766  & 0.475 & 0.766  & 0.067 & 0.039 & 141.6  & 122   \\
% 		8  & 0.624  & 0.365 & 0.624  & 0.054 & 0.04  & 35.7  & 90     \\ \midrule
% 		9  & 0.641  & 0.466 & 0.641  & 0.056 & 0.045 & 133.3  & 106.3 \\
% 		10 & 0.45   & 0.421 & 0.45   & 0.039 & 0.034 & 69.4  & 110.9  \\
% 		11 & 0.598  & 0.597 & 0.598  & 0.052 & 0.025 & 92.3   & 109.3 \\ \bottomrule
% 	\end{tabular}
% \end{table*}

% \subsection{Inference Strategies}
% Stage-1 training of encoder and decoder with affine layers.

% \subsection{large and diverse dataset}
% Qualitative results
% \subsection{Evaluation Metrics}

% SSIM (higher the batter),
% PNSR (higher the batter),
% Datasets and Implementation.

% Comparisons with Prior Works 

% Limitations: maintaining the dimensions to follow the Normalizing Flow methods.

% \subsection{Comparison with Existing Methods} We evaluate our proposed model on the two real image datasets (DIV2K-valid, RealSR) and one generated image dataset (DrealSR) with high and low-resolution pairs.  Performance comparison between our approaches and several other methods on two benchmark datasets. PSNR/SSIM values on the Y channel are reported on each dataset. \#Ps and FLOPs stand for the total number of network parameters and floating-point operations, respectively. FLOPs are measured under the setting of upscaling SR images to 256×256 resolution on the $\times2$ scale.

% \begin{figure}[!pht]
%         \centering
% 	% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
% 	\includegraphics[width=0.991\linewidth ]{figures/val_loss_affineAE_vs_AEKL.png}
% 	\caption{Val total loss (rec-loss, nll-loss, and ae-loss) plot affine-AE vs AE-KL for training 50 epochs.}
% 	\label{fig:affineAE_vs_AE_loss}
% \end{figure}

% \vspace{-2em}



% \subsection{Future work}

% Sampling time.\
% Guided SR.\
% Text and image as input. \
%In this paper, we train the practical Real-ESRGAN for real-world blind super-resolution with pure synToning pairs. We propose a high-order degradation process to synthesize more practical degradations and employ sinc filters to model common ringing and overshoot artifacts. We also utilize a U-Net discriminator with spectral normalization regularization to increase discriminator capability and stabilize the training dynamics. Real-ESRGAN trained with synthetic data can enhance details while removing annoying artifacts for most real-world images.
%fast, small, more training params. Two-stage training,

% Stage-1 training of encoder and decoder with affine layers.


%%% Chapter-9


%%% Chapter-12

% This thesis proposal has significantly contributed to both the theoretical foundations of generative models and their practical applications in computer vision. Our work spans two significant directions: advancing the efficiency of normalizing flow models and applying generative modeling techniques to solve real-world problems. Indomain of flow-based models, we introduced CInC Flow and Inverse-Flow. This novel architecture is significantly state-of-the-art through several key innovations, including the development of an efficient backpropagation algorithm for inverse convolution optimized for parallel operations, the implementation of a multi-scale architecture that substantially accelerates sampling in normalizing flow models, and the creation of a CUDA-based GPU implementation that enhances computational performance. Comprehensive experimental validation has demonstrated improved training capability and sampling speed compared to existing approaches.

% Our applications of generative models to computer vision problems have yielded significant results across multiple domains. In geological mapping, we demonstrated the effectiveness of stacked autoencoders combined with k-means clustering, achieving superior feature extraction compared to traditional methods. Framework's integration with Sentinel-2 data yielded the highest spatial resolution and accuracy, particularly in the Motawintji region of NSW, Australia. For image super-resolution, we developed Affine-StableSR, which successfully addresses computational and model size challenges through integration of affine-coupling layers in encoder-decoder architectures, efficient utilization of pre-trained weights from stable diffusion models, and introduction of a diverse four-in-one dataset for robust training. 

% In art restoration, we advanced the field by adapting diffusion models for comprehensive image restoration, developing systematic fine-tuning processes, creating a taxonomy of ten distinct distortion types, and conducting comparative assessments of existing methodologies across multiple restoration tasks. Our approach demonstrated superior performance in handling various degradation through unified fine-tuning, making it particularly valuable for cultural heritage preservation.

% \section{Future Work}

% Looking ahead, several promising research directions emerge from this work. We plan to explore enhanced convolutional inversion models, particularly for atmospheric effect modeling, and expand privacy-preserving capabilities for autonomous driving applications. Developing more robust face and license plate detection systems and extending our methods to broader stable diffusion applications remains a priority. Additionally, we aim to refine training strategies for diffusion model-based image restoration, focusing on specialized datasets for distinct degradation types.

% This work establishes a strong foundation for future advancements in efficient generative modeling and its applications, contributing significantly to computer vision, geological mapping, image enhancement, and art restoration. Frameworks and methodologies developed here offer promising pathways for continued innovation in these domains, particularly in addressing real-world challenges where computational efficiency and accuracy are paramount.

% This thesis proposal has made significant contributions to both the theoretical foundations of generative models and their practical applications in computer vision. Our work spans two major directions: advancing the efficiency of normalizing flow models and applying generative modeling techniques to solve real-world problems.

% Indomain of flow-based models, we introduced Inverse-Flow, a novel architecture that is significantly state-of-the-art through several key innovations:
% - Development of an efficient backpropagation algorithm for inverse convolution, optimized for parallel operations
% - Implementation of a multi-scale architecture that substantially accelerates sampling in normalizing flow models
% - Creation of a CUDA-based GPU implementation that enhances computational performance
% - Comprehensive experimental validation demonstrating improved training capability and sampling speed

% Our applications of generative models to computer vision problems have yielded significant results across multiple domains:
% 1. In geological mapping, we demonstrated the effectiveness of stacked autoencoders combined with k-means clustering, achieving superior feature extraction compared to traditional methods. Framework's integration with Sentinel-2 data yielded the highest spatial resolution and accuracy, particularly in the Motawintji region of NSW, Australia.

% 2. For image super-resolution, we developed Affine-StableSR, which successfully addresses computational and model size challenges through:
%    - Integration of affine-coupling layers in encoder-decoder architectures
%    - Efficient utilization of pre-trained weights from stable diffusion models
%    - Introduction of a diverse four-in-one dataset for robust training

% 3. In art restoration, we advanced by:
%    - Adapting diffusion models for comprehensive image restoration
%    - Developing systematic fine-tuning processes
%    - Creating a taxonomy of ten distinct distortion types
%    - Conducting comparative assessments of existing methodologies across multiple restoration tasks

% Looking ahead, several promising research directions emerge:
% 1. Further exploration of enhanced convolutional inversion models, particularly for atmospheric effect modeling
% 2. Expansion of privacy-preserving capabilities for autonomous driving applications
% 3. Development of more robust face and license plate detection systems
% 4. Extension of our methods to broader stable diffusion applications
% 5. Refinement of training strategies for diffusion model-based image restoration

% This work establishes a strong foundation for future advancements in efficient generative modeling and its applications, contributing significantly to fields of computer vision, geological mapping, image enhancement, and art restoration. Frameworks and methodologies developed here offer promising pathways for continued innovation in these domains.


% In this thesis proposal, we introduced Inverse-Flow, a novel flow-based model that uses a fast and efficient backpropagation algorithm specifically designed for inverse of convolution, leveraging convolutional operations to enable efficient sampling and learning. Our contributions to generative modeling include:

% \paragraph{Efficient Backpropagation:} We developed a backpropagation algorithm for inverse convolution optimized for parallel and independent operations, improving training speed and sampling efficiency.
% \paragraph{Multi-Scale Architecture:} Inverse-Flow's multi-scale design significantly accelerates sampling in normalizing flow models.
% GPU Implementation: A CUDA-based GPU implementation of Inverse-Flow and its backpropagation algorithm was created, enhancing computational performance on modern hardware.
% \paragraph{Experimental Validation:} Comprehensive experiments demonstrate Inverse-Flow's strong training capability and substantial sampling speed improvement compared to traditional flow models.
% These results confirm that the inverse of convolution can be effectively trained and utilized for both sampling and training, with Inverse-Flow significantly improving sampling time for normalizing flow models. This positions flow-based models as competitive with other generative techniques, such as GANs, diffusion models, and vision transformers. The backpropagation algorithm for inverse convolution opens new possibilities for developing faster, more expressive flow-based models with broad applications across computer vision and other fields.

% \section{Future Work}
% Future directions of this work include expanding the scope of invertible convolution and enhancing privacy-preserving capabilities for autonomous driving applications:

% \paragraph{Enhanced Convolutional Inversion Models:} Further exploration of atmospheric effects on Hermite and Laguerre Gaussian beams, particularly under different conditions, will refine accuracy in long-range propagation modeling. Additionally, multi-channel atmospheric propagation effects will be examined in future models.

% \paragraph{Face and License Plate Detection:} Building on our findings, we plan to refine YOLOX architecture, creating a more robust baseline model for detecting faces and license plates in autonomous driving, even without labeled data. This model aims to outperform generic state-of-the-art systems and will undergo in-depth failure analysis to identify current limitations and inform future developments.

% \paragraph{Expanding Pvt-IDD Dataset:} We aim to broaden Pvt-IDD to include diverse real-world scenarios for enhanced privacy-preserving technology. Recognizing potential ethical risks, such as bias propagation from large vision models, we will explore rule-based filtering and tailored classifiers to minimize harmful data, ensuring responsible and equitable use of autonomous driving technologies.

% This work set the stage for significant advances in efficient flow-based models and real-world applications, contributing to generative modeling, privacy preservation, and autonomous driving fields.

% \paragraph{Generative Model and Image Dimension Reduction}
% We presented a framework that combined stacked autoencoders with $k$-means clustering to generate geological maps. By applying various pairs of remote sensing data types and dimensionality reduction methods, we created input features for the for$k$-means algorithm, resulting in automated geological maps for the forMutawintji region in NSW, Australia. Our investigation revealed that combining stacked autoencoders with Sentinel-2 data yields the highest spatial resolution and accuracy compared to other combinations. Stacked autoencoders were highly effective for dimensionality reduction and feature learning, enabling better extraction of complex and hierarchical representations of input data compared to canonical autoencoders and PCA. Our findings reveal that the integration of stacked autoencoders with Sentinel-2 data yields the highest spatial resolution and accuracy. Stacked autoencoders proved to be highly effective for dimensionality reduction and feature learning, enabling extraction of more complex and hierarchical representations of input data compared to canonical autoencoders and PCA.flexibility of our framework allows for further enhancements with incorporation of novel dimensionality reduction and clustering methods. This adaptability ensures that our approach can evolve alongside advancements in remote sensing and machine learning techniques, making it a robust tool for geological mapping in various regions and contexts.

% \paragraph{ Generative Models and Image Super-resolution}
% This work introduces Affine-StableSR, a novel approach harnessing diffusion priors for real-world Super-Resolution (SR). We undertake targeted training of both encoder and decoder from scratch, addressing prevalent challenges such as high computational demands and model size. Our proposed solutions incorporate affine-coupling layers with encoder and decoder architectures. We envision our contributions as foundational steps in this domain, with Affine-StableSR offering valuable insights for future research amalgamating concepts from normalizing flows and diffusion models. Furthermore, we present the Affine-StableSR framework, integrating encoder and decoder structures with affine-coupling layers and pre-trained weights for a stable diffusion model. Leveraging pre-trained weights from the StableSR for diffusion model (U-net), we introduce a new four-in-one dataset comprising images from four distinct sets to enhance training image diversity. We foresee the potential extension of our method to stable diffusions, such as replacing resnet block of U-net and even transformer for vision tasks.
% \paragraph{ Generative Models and Image Art Restoration}
% In conclusion, this endeavor has spotlighted the efficacy of contemporary diffusion models in the realm of image restoration (IR), harnessing their robust generative potential to amplify both structural and textural revitalization. The initial phase of this work entailed leveraging pre-trained weights to establish a foundational baseline, followed by a progressive evolution of the diffusion model for IR applications, with a specific focus on the adaptation of StableSR, through a systematic fine-tuning process. This research has further delved into the comprehensive categorization of ten distinct distortions, shedding light on their nuances through the lens of training strategies and degradation scenarios.

% Through meticulous analysis, we undertook a comparative assessment of existing works, encompassing both super-resolution and IR domains. Each approach was dissected precisely, affording an intricate taxonomy delineating their respective strengths and weaknesses. The evaluation process involved an overview of prevalent datasets and evaluation metrics within a diffusion model-based IR landscape. This culminated in a comprehensive comparison of two cutting-edge open-source state-of-the-art (SOTA) methodologies, evaluated through a fusion of distortion and perceptual metrics across three quintessential tasks: image super-resolution, deblurring, and inpainting.

% Remarkably, our observations highlighted the effectiveness of training diffusion models on specialized datasets tailored to distinct degradation types. This strategy yielded commendable outcomes, particularly in scenarios mirroring noise or degradation patterns akin to training data. As we steer toward future prospects, addressing challenges inherent in diffusion model-based IR entails exploring diverse baseline datasets and refining training strategies. By doing so, the realm of diffusion models can be further optimized for achieving superior outcomes, marking a promising direction for future exploration. 


% We give a fast and efficient backpropagation algorithm for the inverse of convolution. We proposed a flow-based model, Inverse-Flow, that leverages convolutions for efficient sampling and inverse of convolution for learning. Our work makes several key contributions field of generative modelling:

% \begin{enumerate}
%     \item We proposed a fast backpropagation algorithm for the inverse of convolution, leveraging independence and parallelization operations to improve fast training with faster sampling.
%     \item We developed a multi-scale Inverse-Flow architecture that significantly accelerates the sampling process in flow models. 
%     \item We provided a GPU (CUDA) implementation of Inverse-Flow and its corresponding backpropagation algorithm, enabling high-performance computation on modern hardware.
%     \item We conducted extensive experiments to demonstrate the training capabilities of inverse flow and its substantial improvements in sampling time compared to traditional flow models.
% \end{enumerate}

% In this thesis proposal, Inverse-Flow implementation shows proof that the inverse of convolution can be trained and used for sampling and inference.GPU implementation of backpropagation for inverse convolution fast training and faster sampling using flow-based model architecture. We show a big improvement in sampling time for normalizing flow models and outflow models in competition with other generative models such as Diffusion, GANs, and Vision transformers. Backpropagation algorithm algorithm forinverse convolution a new set of possibilities for training fast and more expressive Flow models. 

% Our results demonstrate thatinverse of convolution can be effectively trained and utilized for both sampling and training.GPU implementation of backpropagation for the inverse of convolution facilitates rapid training and significantly faster sampling with inflow-based model architecture. Notably, we achieved substantial improvements in sampling time for normalizing flow models and positioning flow-based approaches as competitive alternatives to other generative models such as diffusion models, GANs, and vision transformers. Furthermore, our efficient backpropagation algorithm for inverse convolution opens new possibilities for training more expressive and fast-flow models. This advancement has the potential to broaden the applicability of flow-based models across various domains in computer vision and beyond. 

% \section*{Future works}

% Some other atmospheric effects under different conditions on Hermite and Laguerre Gaussian need to be modeled for more accurate results in long-range propagation in atmospheric turbulence. We are investigating the effects of multi-channel propagation in the atmosphere on an adjacent beam. We plan to experimentally set up a system for low-power lasers to verify the designed system.

==> FrontMatter/abbreviations.tex <==
\thispagestyle{plain}
\begin{center}
    \huge \textbf{List of Abbreviations}
\end{center}



\vspace{\baselineskip}

\justifying


\begin{acronym}[BDOC]
    % \acro{BC}{Beam combination}
    % \acro{BCS}{Beam combination system}
    % \acro{CBC}{Coherent beam combination}
    % \acro{SBC}{Spectral beam combination}
    % \acro{IBC}{incoherent beam combination}
    % \acro{HG}{Hermite Gaussian}
    % \acro{LG}{Laguerre Gaussian}
    % \acro{BG}{Bessel Gaussian}
    % \acro{BDOC}{beam directing optical channel}
    % \acro{MOPA}{master oscillator power amplifier}
    % \acro{FTB}{fiber-tapered bundles}
    % \acro{PTR}{Photo-thermo-refractive}
    % \acro{AFOC}{adaptive fiber-optics collimators}
    % \acro{SPGD}{stochastic parallel gradient descent}
    % \acro{BPE}{Beam propagation efficiency}
    % \acro{BPP}{beam parameter product}
    % \acro{MMF}{multi-mode fiber}
    % \acro{SMF}{single-mode fiber}
    % \acro{FMF}{few-mode fiber}
    % \acro{SMFe}{Single-Multi-Few mode device}
\end{acronym}





==> FrontMatter/disclaimer.tex <==
\thispagestyle{plain}

\begin{center}
 \Large {\bf \uppercase{Disclaimer}}
\end{center}

\vspace{3\baselineskip}

\justifying
\noindent
This thesis represents research that has been carried out by me (and some collaborative work), including some work in progress.



==> FrontMatter/symbols.tex <==
\thispagestyle{plain}
\begin{center}
    \huge \textbf{List of Symbols and Notations}
\end{center}


\vspace{\baselineskip}

\justifying

\begin{tabular}{p{1.5cm} p{8cm}}
    % $N$ & No of Laser source \\
    % $\lambda$ & Wavelength \\
    % $h$ & Altitude height \\
    % $P$ & Power \\
    % $k$ & Wave number \\
    % $v_x$ & Wind speed \\
    % $L$ & Propagation distance \\
    % $f$ & Focal length of collimating lens\\
    % $W_0$ & Initial spot size \\
    % $W(z)$ & Spot size at $z$ distance \\
    % $\alpha$ & Tilt angle \\
    % $I_0$ & Initial peak intensity \\
    % $\epsilon$ &  Total extinction coefficient \\
    % $S_{atm}$ & Atmospheric Strehl Ratio \\ 
    % $S_{jitter}$ & Jitter Strehl Ratio \\
    % $S_{TB}$ & Thermal blooming Strehl Ratio \\
    % $W_d$ & Spot size variation due to diffraction \\
    % $W_j$ & Spot size variation due to jitter \\
    % $W_t$ & Spot size variation due to turbulence \\
    % $r_0$ &Fried parameter \\
    % $N_D$ & Thermal distortion number \\
    % $C_p$ & Specific heat of air \\
    % $\alpha(z)$ & Absorption coefficient \\
    % $\beta$ & Scattering coefficient \\
    % $C_n^2$ & Atmospheric turbulence \\
    % $\eta$ & Efficiency \\
    % $\rho_0$ & Bucket spot radius \\
    % $\sigma_R^2$ & Rytov parameter \\
    
\end{tabular}



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% \usepackage{nicematrix}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

